A Methodology for the Offline Evaluation of Recommender Systems in a User Interface with Multiple Carousels

Many video-on-demand and music streaming services provide the user with a page consisting of several recommendation lists, i.e. widgets or swipeable carousels, each built with a specific criterion (e.g. most recent, TV series, etc.). Finding efficient strategies to select which carousels to display is an active research topic of great industrial interest. In this setting, the overall quality of the recommendations of a new algorithm cannot be assessed by measuring solely its individual recommendation quality. Rather, it should be evaluated in a context where other recommendation lists are already available, to account for how they complement each other. This is not considered by traditional offline evaluation protocols. Hence, we propose an offline evaluation protocol for a carousel setting in which the recommendation quality of a model is measured by how much it improves upon that of an already available set of carousels. We report experiments on publicly available datasets on the movie domain and notice that under a carousel setting the ranking of the algorithms change. In particular, when a SLIM carousel is available, matrix factorization models tend to be preferred, while item-based models are penalized. We also propose to extend ranking metrics to the two-dimensional carousel layout in order to account for a known position bias, i.e. users will not explore the lists sequentially, but rather concentrate on the top-left corner of the screen.

==> main-body.tex <==


\section{Introduction}
% \mf{bozza}
Video on demand and music streaming services are among the most successful application domains of Recommender Systems. %The research and industry communities are constantly at work to develop new and ever more effective algorithms. 
Often, in a video-on-demand service (\eg Netflix, Amazon Prime Video) or on a music streaming platform (\eg Spotify) the user is provided with multiple rows of recommendations, each generated according to a specific criterion, \eg most recent, most popular, editorially curated (see Figure \ref{fig:amazon_netflix}). These rows are referred to as \emph{widgets}, \emph{shelves} or as \emph{carousels}.
%if the user has the ability to swipe them and reveal further items.
In this scenario, the user satisfaction and behavior does not depend on a single recommendation list but rather on the entire set of recommendations provided in the various carousels, as well as their position. Finding appropriate combinations of algorithms and ranking them to provide the user with a personalized page is an active research topic of significant industrial interest  \cite{DBLP:conf/recsys/BendadaSB20,DBLP:conf/kdd/DingGV19,DBLP:conf/recsys/WuASB16}.



% When developing a new algorithm there are two main opinions for its evaluation: \emph{online} and \emph{offline}. Online evaluation is usually performed with A/B testing, where some users interact with the previous system and others with the new one. Online evaluation allows to measure the real impact on the user behavior and satisfaction, however it has significant limitations, namely it requires to integrate the proposed approach into a platform with real users, which is time consuming and expensive.

% Due to these limitations, most analysis are based on \emph{offline evaluation}, by training and testing the proposed approach on a dataset of previously collected interactions. It is known that offline evaluation can often lead to different results than \emph{online evaluation}, this is due to several factors \mf{ref}, among which that the historic data contains interactions which are mediated by the recommender system used by the service which collected them, but also user interface bias which will impact the user exploration...

% Due to how expensive it is to run \emph{online evaluation}, or A/B testing, on real user, offline experiments remain crucial to prune all the possible strategies in order to test with real users only the most promising ones.
% It is therefore very important to ensure that the offline evaluation scenario mirrors as closely as possible the real one.
% In most video-on-demand and many music streaming services content is organized in multiple rows of recommendations, each generated according to a specific criteria (\eg most recent, most popular, editorially recommended). These rows are referred to as \emph{widgets} or \emph{shelves} or as \emph{carousels} if the user has the ability to swipe them and reveal further items.

Despite this, in the traditional offline evaluation scenario each recommendation model is evaluated independently and the one with the highest quality is preferred. This evaluation procedure does not take into account how would the different recommendation lists complement each other in a real carousel user interface. As a consequence, it may lead to the selection of algorithms that provide similar sets of recommendations.
%, \eg may concentrate on popular items if the dataset is popularity biased. %This is an undesired result, since 
Since it is known that a set of diverse recommendations improves user satisfaction \cite{chen2018fast}%,DBLP:conf/recsys/ZhangH08}
, and recommending the same item in multiple lists has little use, in some cases it will be beneficial to include algorithms with a lower individual recommendation quality if they generate recommendations with a different perspective.
% with a different perspective, even if their individual recommendation quality is lower.
Most articles targeting recommendations in a carousel setting are evaluated online with users of a certain platform. This puts a high resource requirement on researchers which will limit their ability to investigate this scenario. 
Furthermore, 
%as will be discussed later,
there seems to lack a standardized evaluation protocol to allow for offline experiments in a carousel setting. This is true, in particular, for how the two-dimensional structure of the user interface is taken into account in ranking metrics for which, to the best of our knowledge, no offline metric exists.
% As an extreme example we can imagine a scenario where the dataset is very popularity unbalanced and a non personalized model provides a better recommendation quality than other personalized models. In a traditional offline valuation protocol this would indicate the non personalized model to be the best option. In a real scenario where multiple models are shown to the user even a lower performing model can be added if it complements the top pop \mf{orribile}
% The goal in this case is not how well a model performs by itself, but rather how well it performs in conjunction with other ones. 
% It is known that the user behavior is influenced by how the different widgets are organized in the page and developint algorithms to sort them is an active research topic \mf{ref}
% These approaches however are mainly evaluated with A/B testing. The offline evaluation are done usually by ranking all the recommendations generated by the different models as a slingle list or .... \mf{vedere}

To address the highlighted issues, in this paper we propose a novel offline evaluation protocol that closely mirrors a real user interface with multiple carousels. In this setting, the recommendation quality of each model is computed by how much it improves the accuracy over one or more fixed carousels, in order to better evaluate the user satisfaction in such scenario. The contributions of this paper are as follows:
\begin{itemize}
    \item We propose an offline evaluation protocol based on real industrial carousel settings and provide experimental results highlighting the different relative accuracy of models evaluated in this way;
    % upon the carousel user interface for 
    %video-on-demand
    %or music streaming 
    %services;
    \item We extend the widely used NDCG metric \cite{DBLP:conf/sigir/JarvelinK00}
    to a two-dimensional layout, that takes into account the user exploration behavior while navigating carousels. To the best of our knowledge, there exists no ranking metric that takes into consideration a two-dimensional layout.
    %\item We compare the recommendation quality of several widely known algorithms when evaluated independently and in a carousel setting, highlighting their different relative accuracy;
    % \item We discuss how the carousel evaluation protocol rewards the selection of diverse recommendation lists.%, which is consistent to what observed in previous A/B tests that diverse recommendations improve user satisfaction. 
\end{itemize}

% \nico{Tolto dalle contributions il fatto che abbiamo condotto esperimenti e comparato individual con carousel setting. Va bene?} 
The rest of the paper is organized as follows. Section \ref{sec:related_works} presents related works on carousel interfaces. Section \ref{sec:evaluation_protocol} provides a description of the carousel scenario and
%how
%both ranking, accuracy and beyond-accuracy  \nico{forse da togliere le beyond acc} 
%metrics should be computed.
the evaluation protocol.
Section \ref{sec:experimental_anaysys} reports the results of our experimental analysis. Finally, Section \ref{sec:conclusions} draws conclusions and presents possible future works.



% \nico{some UMAP keywords: personalization and adaptation, user modeling and adaptation, recommender systems, adaptive educational systems, intelligent user interfaces, e-commerce, advertising, digital humanities, social networks, personalized health, entertainment}

% \nico{ As the theme for UMAP 2021 is “Re-Evaluating Evaluation” we encourage submissions in all areas that offer a critical analysis of evaluations of personalized systems.}


% \begin{figure*}[]
%     \centering
%     \begin{minipage}{.49\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{images/amazon_2048_1380.PNG}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.49\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth]{images/netflix_2048_1380.jpeg}
%     \end{minipage}
%     \caption{Examples of carousel user interfaces in the multimedia streaming domain. On the left, there is the Amazon Prime Video homepage, while on the right, there is the Netflix homepage.}
%     \label{fig:amazon_netflix}
% \end{figure*}

\begin{figure*}[]
    \centering
    \begin{minipage}{.45\textwidth}    
        \centering
        \includegraphics[width=1.\textwidth]{fig01.jpeg}
        \caption{The Netflix homepage, an example of carousel user interface in the multimedia streaming domain.}
        \label{fig:amazon_netflix}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1.\textwidth]{fig02.pdf}
        \caption{Heatmap of the number of interactions per position on the screen, taken from
        the dataset presented in 
        \cite{DBLP:conf/cikm/MaureraDSSC20}. 
        %Values are log-scaled.
        }
        \label{fig:cw_heatmap}
    \end{minipage}
\end{figure*}








\section{Related Work}
\label{sec:related_works}
Most of the works targeting a carousel user interface come from industrial research. 
This demonstrates the importance, at the industrial level, of identifying an adequate combination of carousels to show to the user.
However, it may also indicate that the lack of a standardized offline evaluation protocol is hampering researchers who do not have easy access to online evaluation infrastructure, preventing them to work on the topic.

% How to handle recommendations in a user interface with a two-dimensional layout is a widely known problem in the research area of recommender systems. 

\citet{DBLP:conf/recsys/WuASB16} analyze the problem of optimizing the position of the carousels on the interface of Netflix, a popular online video streaming service. %The homepage of Netflix is personalized and has a two-dimensional layout. The authors call  \textit{row} a set of thematically coherent videos, and the homepage is composed of a set of rows.
%Therefore, their objective is both to optimize the ranking of the rows and to optimize the ranking of the videos within each row. 
The authors propose a graphical model based on the notion that the benefit of recommending a certain item depends on how novel it is relatively to the previous recommendations, a concept referred to as \textit{submodularity}. Their algorithm is able to leverage scrolls and navigation feedback to dynamically optimize the user interface. The evaluation is done both online and offline. For the offline evaluation standard metrics are reported (MRR and Precision) considering a carousel as a single item which is relevant if it contains at least a relevant recommendation, therefore not accounting for the ranking within the carousel. %\mf{verificare}
% Our objective, instead, is to make an offline evaluation of the user experience with such a layout. Also, we consider constraints applied to the user interface due to business decisions, which were not considered in this paper. 
% In \cite{DBLP:conf/recsys/WuASB16}, the authors analyse the problem of optimizing the position of the recommended videos on the interface of Netflix, a popular online video streaming service. The homepage of Netflix is personalized and has a two-dimensional layout. The authors call  \textit{row} a set of thematically coherent videos, and the homepage is composed of a set of rows. Therefore, their objective is both to optimize the ranking of the rows and to optimize the ranking of the videos within each row. They propose a graphical model based on the notion of \textit{submodularity}. In their scenario, the submodularity property translates to the fact that the benefit of recommending an item does not depend on that item in isolation, but instead on how novel it is relatively to the previous recommendations. This reasoning is sound, especially in our scenario where duplicates in different rows are allowed, and it is the basis of our novel evaluation approach. The main focus of this paper, though, is including scrolls and navigation feedback of the user in real-time to dynamically optimize the interface in an online fashion. Our objective, instead, is to make an offline evaluation of the user experience with such a layout. Also, we consider constraints applied to the user interface due to business decisions, which were not considered in this paper. 
\citet{DBLP:conf/wsdm/GrusonCCMHTC19} optimize the homepage of Spotify, an online music streaming service.
%, which recommends playlists in thematic rows referred to as \textit{shelves}.
The paper evaluates a series of policies to rank the most relevant playlists for a user. The policies are ranked according to first an online evaluation and then an offline evaluation. The two rankings are then compared and de-biasing techniques are discussed to improve the correspondence of offline evaluations with online ones.
% The objective of this paper is to learn a policy that ranks the most relevant playlists for a user in an offline way and then test online the obtained policy. To do so, they rely on the knowledge of the logging policy, which, instead, we can not exploit. Also, they assume the same policy to be used to recommend the whole homepage. 
In the offline evaluation, the carousels are sequentially concatenated as a single long recommendation list. This evaluation procedure, however, does not take into account the behavior of a user while exploring a two-dimensional interface. Again, the article points out at discrepancies between the online and offline evaluations.
%Essentially, they treat a set of $s$ shelves, composed of $p$ playlists each, as a global ranking \mf{cosa vuol dire?} \nico{nel paper assumono che la homepage sia il risultato di un singolo modello con cutoff s x p, noi invece consideriamo il caso in cui ogni riga sia il risultato di un algoritmo diverso} problem of $s \cdot p$ playlists. This is different from our approach because, in real scenarios, rows must be thematically coherent, to ease user navigation. Therefore, different rows are usually the results of different algorithms. 
% The evaluation is done based on the \textit{importance sampling} technique \cite{horvitz1952generalization}, which relies on the knowledge of the original recommendation policy used. 
% Interestingly, they found several discrepancies between the online and offline results, which may suggest the necessity of a novel evaluation protocol that is more consistent with a real-world setting. 
% For instance, there may be editorial constraints on which row to show on the interface, which are not taken into account in this paper.
% In \cite{DBLP:conf/wsdm/GrusonCCMHTC19}, the authors face the problem of optimizing the homepage of Spotify, an online music streaming service. Such homepage, similar to Netflix's one, is composed of rows, which are called \textit{shelves} by the authors. Each shelf is composed of a set of playlists. The objective of this paper is to learn a policy that ranks the most relevant playlists for a user in an offline way and then test online the obtained policy. To do so, they rely on the knowledge of the logging policy, which, instead, we can not exploit. Also, they assume the same policy to be used to recommend the whole homepage. Essentially, they treat a set of $s$ shelves, composed of $p$ playlists each, as a global ranking problem of $s \cdot p$ playlists. This is different from our approach because, in real scenarios, rows must be thematically coherent, to ease user navigation. Therefore, different rows are usually the results of different algorithms. Furthermore, there may be editorial constraints on which row to show on the interface, which are not taken into account in this paper.
\citet{DBLP:conf/recsys/BendadaSB20} propose a contextual multi-armed bandit online approach to optimize the two-dimensional layout of the homepage of an online music streaming service, called Deezer. Each user is shown a set of carousels which the user can swipe to reveal further items but the system does not log all user actions. To estimate which items the user has seen in the hidden part of the carousels they rely on the \textit{cascade model} \cite{DBLP:conf/wsdm/CraswellZTR08} assuming the user has seen all items before the one they interacted with and therefore has swiped and ignored them. The policies are evaluated both online and offline with expected cumulative regrets.
% Specifically, they refer to each row as a \textit{swipeable carousel}, where the length of the carousel is some number $L$, but only $L_{init} < L$ items can be shown in the initial setting of the homepage, due to size limitations. Therefore, this can introduce \textit{position bias} for items that are not shown initially, since they assume there is no information regarding the swiping activity of users. To cope with this issue, the authors propose an approach similar to that of the \textit{cascade model} \cite{DBLP:conf/wsdm/CraswellZTR08}. With this approach, they associate negative feedback from a user to an item not shown initially in the carousel (i.e., ranked with a rank $ i > L_{init}$) only when the user interacts with another item with rank $ j > i$. In this way, they are sure that the user ignored the item $i$ intentionally and not because of the position bias. These complexities are not considered in our work, since we assume rows to be static and not swipeable, but it could be a possible direction for future work. Still, in this paper, the evaluation does not consider the interaction of different carousels and their impact on user experience, which is instead the main focus of our work.
\citet{DBLP:conf/kdd/DingGV19} targets the problem of whole page optimization for the homepage of Amazon Video, a video streaming service. %The user interface of this streaming service is two-dimensional, like the scenario we are considering. The authors call the rows that compose the homepage \textit{widgets}. 
They assume that a set of carousels is already available and that the objective is to select which carousels to show and in which order while also accounting for the business constraints of the homepage. % (\idest rank the widgets). 
% An important aspect of this work is that it is the first to consider the business constraints of the homepage. Therefore, they propose a primal-dual approach that aims to maximize the accuracy of the shown widgets, but subject to the constraints due to business decisions. 
%\nico{Differences: we are only evaluating and not optimizing, business constraints are averaged on the whole user base, we are considering instead a variant of slotting.}
It should be noted that the personalization of homepage is a widely discussed problem also in other domains. For example,
\citet{DBLP:conf/www/AgarwalCYZ15} propose an optimization framework for the personalized widget layout on Linkedin, a known professional social network site, to improve user engagement. As opposed to the video-on-demand or music streaming scenario where there are many carousels available, in \cite{DBLP:conf/www/AgarwalCYZ15} there is only one.
Finally, some works try to account for the two-dimensional structure of the page during the algorithm training phase. For example, \citet{DBLP:conf/recsys/ElahiC20} propose to model the user response to the two-dimensional interface as an embedding.
% model is built for scenarios where users interact with sets of items rather than single items. The authors call the sets of items \textit{slates} and propose a method to learn \textit{slate embeddings}. To do so, they present a \textit{hierarchical approach}, taking into consideration the multiple (spatial or temporal) dimensions of a user interface. 
% In our work, we do not build slate embeddings, but we consider the two-dimensional hierarchy typical of a real-scenario streaming service. \nico{forse da rifare} \nico{capire se e' davvero rilevante}
% \nico{non so se va bene citare esplicitamente i servizi tipo Netflix e Spotify}
% \nico{chiarire che sono proprio i ricercatori dell'azienda}

% Another related line of research is that of \textit{whole page optimization}, typical of the information retrieval domain. \citet{DBLP:conf/wsdm/WangYJWYCM16} first described this issue (and later extended their analysis in \cite{DBLP:journals/tweb/WangYJWYCM18}) applied to the information retrieval field. In particular, they face the problem of deciding how to display a given heterogeneous set of items (links, images, videos, etc.) on the search result page. This problem is called \textit{page presentation optimization}.
% There is no constraint on the layout of the page, therefore they abstract it as a two-dimensional grid, where any item can be placed anywhere in the grid. Finally, they present a novel framework for optimizing the page presentation, learning where to place the items on the page using implicit user feedback. 
% This work highlights the advantages of considering the whole page, instead of the single displayed items in isolation, to enhance the user experience. Nevertheless, it applies only to the information retrieval field. In fact, in our scenario, we consider a constrained layout composed of rows. Also, business constraints can force some rows to be present on the shown page. Finally, we do not consider the heterogeneity of the items to recommend, which is something relevant for the information retrieval scenario. \nico{l'ultima frase non mi convince.}


% \nico{maybe i have to cite also \cite{DBLP:conf/www/AgarwalCYZ15} because it introduces the problem of slotting in LinkedIn} \mf{ci guardo io}
% \citet{DBLP:conf/www/AgarwalCYZ15} propose an optimization framework for the personalized widget layout on Linkedin, a known professional social network site, to improve user engagement. The article discusses in particular the problem of estimating reward and the business constraints.




\section{Carousel Evaluation Characteristics}
\label{sec:evaluation_protocol}
%\nico{non è proprio un protocollo, forse scenario, cambia titolo}
%In this section we describe the proposed carousel evaluation protocol, which aims to closely resemble both a real user interface and a real industrial setting.
% \nico{Non mi convince com'e' formattata questa sezione. c'e' un 3.1 senza un 3.2 e un 3.1.1 senza un 3.1.2} 
In this section we describe the characteristics of a real user interface in an industrial setting using a carousel layout.
\begin{description}
    \item[Interface:] A two-dimensional user interface (\idest a grid of recommendations) composed of different carousels (\idest rows). %They can have the same length, but this is not always the case.
    In the general case, carousels may have different lengths which we assume remain constant for all users.
    % \nico{r2 dice: I am also not convinced with the assumption that all lists have the same length. This is not the case in practice. }
    %\nico{Se le liste sono di dimensioni diverse non è un problema per le metriche di accuracy. Nel caso di NDCG2D possiamo assumere la griglia come numero di carousel X max numero di item per carousel, assumere i buchi come non rilevanti.}
    
    \item[User Behaviour:] The user will not explore the interface one carousel at a time, in a sequential way. Rather, they tend to explore a two-dimensional carousel interface focusing on the top-left corner %\cite{DBLP:conf/etra/KammererG10,
    \cite{DBLP:conf/recsys/ZhaoCHK16}
    (see also Figure \ref{fig:cw_heatmap}). %\nico{forse si possono citare prima} 
    
    \item[Recommendations:] Each carousel is generated with a different algorithm or may come from a different provider, which may know the general layout of the page and the number of carousels, but will be unaware of the specific recommendations contained in the other carousels\footnote{This is common, with \emph{content aggregators} that aggregate carousels from different providers. For instance, a video content aggregator may have a carousels from Sky, Youtube, Netflix, Prime Video, etc.}. In general, no post-processing step is applied. Hence, the same item may be recommended multiple times across different carousels\footnote{For example, in the Netflix homepage shown in Figure \ref{fig:amazon_netflix} the TV series \emph{Space Force} appears both in the \emph{TV Comedies} and \emph{New Releases} carousels.}.
    %Lastly, in order to measure the recommendation quality of the models used to generate one of the baseline carousels, it is sufficient to replicate its recommendation list in all carousels. 
    % \nico{r2 dice: I am not fully convinced about the assumption that model optimization is independent of the UI layout. For instance, the row number of lists in the interface is typically fixed or more stable.} \nico{RISOLTO: detto qui sopra che non si intende indipendente dal layout in se ma dagli altri modelli che comporranno il layout}

    
\end{description}

% \paragraph{Scenario:} The carousel evaluation setting is closely tied to a specific user interface that provides the user with a sequence of recommendation lists, each list (\idest each carousel) generated with a specific model (see Figure \ref{fig:amazon_netflix}). As such, while it could be applied for any domain, we recommend its use be limited to those that employ such carousel interface. Researchers have ample freedom to decide which algorithms to use to generate the carousels. We also recommend that all algorithms used to generate the carousels should be considered and reported as baselines.

% \paragraph{Optimization:} The first step in a comparison between models is to ensure that all are adequately optimized. In a traditional offline evaluation each model is optimized independently by selecting the hyperparameters that optimize its recommendation quality on a validation set \cite{DBLP:conf/recsys/DacremaCJ19}. The same holds for a carousel evaluation. In a carousel setting the recommendation lists provided to the user may come from different sources (\eg a third party providing the recommendation engine for some carousels, while the platform provides others \cite{DBLP:conf/cikm/MaureraDSSC20}), the carousels shown to the user may change dynamically between sessions and different users may see a different carousel selection. This means that during the optimization of the models the layout of the user interface is, in general, not known and cannot be used during the optimization phase. %For this reason, in a carousel evaluation all models will be optimized independently as well.
% For this reason, we will optimize all models independently.

% \paragraph{Recommendation:} The recommendations that will be shown to the users are the sequence of recommendation lists generated by each algorithm. Which algorithms to use and in which order is part of the experimental setting and will be chosen according to the scenario of interest. All lists have the same length, \idest cutoff, $c$. Given $l$ the number of recommendation lists that are displayed, the user will receive $c \cdot l$ recommendations. 
% Moreover, the recommendations may come from different providers which may be unaware of the recommendations contained in the other carousels.\footnote{This is common, with \emph{content aggregators} that aggregate carousels from different providers. For instance, a video content aggregator may have a carousels from Sky, Youtube, Netflix, Prime Video, etc.}
% In general, there will be no postprocessing done on the set of all recommendation lists. 
% While a carousel will only contain a certain item at most once, there could be items appearing in more than one carousel.\footnote{For example, in the Netflix homepage shown in Figure \ref{fig:amazon_netflix} the movie \emph{Space Force} appears both in the \emph{TV Comedies} and \emph{New Releases} carousels.} Lastly, in order to measure the recommendation quality of the models used to generate one of the baseline carousels, it is sufficient to replicate its recommendation list in all carousels.

% \paragraph{Evaluation:} In a carousel setting the recommendations provided to the user will be displayed with a two-dimensional pattern. A frequent simplification is to concatenate all $l$ recommendation lists in a single one of length $c \cdot l$. While this allows to use traditional metrics, it has an important limitation because it does not take into account how the user explores a two-dimensional space. In fact, the user will not explore a list sequentially, but rather start from the top left corner and will move in both directions exploring multiple carousels (see Figure \ref{fig:cw_heatmap}). 
% There may also be items that appear in more that one carousel. When this happens, we must ensure that a correct recommendation is only counted once and with the correct ranking, despite having appeared multiple times in different positions. 
% A detailed description of how the evaluation metrics should be computed is provided in Section \ref{sec:evaluation_metrics}.


% \mf{Bande: TopPop, TopRated, Appena usciti}
% \mf{10 film dell'attore più popolare, del secondo ecc..}
% \mf{Dataset di tipo video e spotify}


\subsection{Evaluation metrics}
\label{sec:evaluation_metrics}
% In this section we describe the evaluation protocol for the carousel evaluation.
% The recommendation lists of the algorithms in the carousel are concatenated with the same ordering as the algorithms. This results in a recommendation list of $c \cdot r$, where $c$ is the cutoff and $r$ the number of algorithms.
% In a real scenario, each algorithm is trained and optimized independently, therefore the recommendations provided by one are not modified according to those provided by another algorithm (\eg the list may contain duplicate recommendations).
% Note that in a real scenario the recommended items would be presented to the user in a bi-dimensional interface and the user exploration of them is not perfectly sequential, rather it is concentrated in the top left corner and decreases both to the right and to the bottom. \mf{figure?} \mf{future developement?} \nico{o qui o nell'intro citare \cite{DBLP:conf/cikm/MaureraDSSC20} ContentWise}
Evaluation in a carousel setting presents broad similarities with a traditional top-n recommendation scenario. An important difference is the presence of duplicates in the recommendation list and the two-dimensional way users explore the interface, which impacts how ranking metrics may consider the item position. %, in the carousel evaluation the recommendation list can contain duplicates, for this reason an appropriate evaluation procedure must be put in place to take that into account. 
In a carousel evaluation scenario, an item in the recommendation list is relevant, \idest a correct recommendation, if it meets two conditions:
\begin{itemize}
    \item The item appears in that user's ground truth
    \item The item has been recommended only once or, if it has duplicates, it is the one corresponding to the \emph{best ranking}. 
    For traditional top-n ranking with a single recommendation list, duplicates are removed from the list; therefore, we assume that each carousel does not contain duplicates. However, duplicates might occur between carousels. Such duplicates must not be removed during the evaluation, in order to mimic the real behavior of carousel-based user interfaces.
    Accuracy metrics are not sensitive to the ranking of items; as such, their measurement with carousel-based used interfaces is the same as with traditional single-list recommender systems.
    %For the same reason, the fact that not all the carousels have the same length does not impact those metrics.

    On the other hand, in order to account for the two-dimensional user exploration of the interface a different definition of ranking discount is needed, as described in Section \ref{sec:two_dim_NDCG}.
\end{itemize}

%\nico{bozza: Another characteristic of the carousel scenario is that not all the recommendation lists have the same length, but this does not impact accuracy metrics.}
%\nico{bozza: Notice how the fact that not all the recommendation lists have the same length does not impact accuracy metrics.}


\subsubsection{Two-dimensional NDCG}
\label{sec:two_dim_NDCG}
The idea of defining a two-dimensional ranking metric stems from the observation that users do not explore each carousel sequentially, but rather start from the top-left corner of the screen and proceed to explore the recommendations both to the right and to the bottom. This behavior has been known for many years in the Information Retrieval field and has been widely researched \cite{DBLP:conf/wsdm/ChierichettiKR11}. 
%Figure \ref{fig:ir_positionbias} shows an example of how the users will tend to focus their attention on a triangle at the top-left corner of a simple user interface.
Understanding how the user attention varies with more complex interfaces is an active research field but is beyond the scope of this paper. The same phenomenon can be observed for recommender systems with a carousel interface. Figure \ref{fig:cw_heatmap} shows the number of interactions for items displayed in the carousel interface of a video-on-demand service, we can again see how the user interactions are concentrated in the  top-left corner \cite{DBLP:conf/cikm/MaureraDSSC20}.
%Due to this, there tend to exist multiple positions which will share a similar position bias. 
%The specific position bias exhibited in a platform depends on several factors, mainly the user interface. It is known, for example, that users are more inclined to swipe carousels if this can be done on a mobile device with a touch, but less so if they are on a desktop computer which requires them to use a mouse. Furthermore, different devices may show a different number of items and carousels. As an example of bias, in Figure \ref{fig:cw_heatmap}, we can see that there is a demarcation between the first and the second half of the columns, which probably is due to one of such user interface biases.
To the best of our knowledge, no ranking metric that takes this behavior into account exists. As a way to approximate this behavior, we propose to extend the commonly used NDCG to the two-dimensional interface. We call this metric \emph{NDCG2D}, which will weight the item position approximating the two-dimensional position bias.
% (see Figure \ref{fig:dcg2d_heatmap}). 

Traditional NDCG is defined as $NDCG = DCG/IDCG$ where DCG is the \textit{Discounted Cumulative Gain} computed from the ranking of the relevant items in the recommendation list and IDCG is the \textit{Ideal Discounted Cumulative Gain} defined as the DCG of the ideal ranked list, \idest the list composed of all the user's relevant items that can fit in the recommendation list length, ranked according to the ground truth relevance. Given $c$ as the cutoff, \idest recommendation list length, $rel(i)$ as the relevance of the item in position $i$, DCG can be computed as shown in Eq. \ref{eq:dcg}.
%follows:

\begin{figure*}
    \begin{minipage}{0.45\textwidth}
        \begin{equation}
        \label{eq:dcg}
            DCG = \sum_{i=1}^{c} \frac{2^{rel(i)} - 1}{log_2(i+1)}     
        \end{equation}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
        \begin{equation}
        \label{eq:dcg2d}
            DCG2D = \sum_{i=1}^{l} \sum_{j=1}^{c}  \frac{2^{rel(i,j)} - 1}{log_2(\alpha i+ \beta j)}
        \end{equation}
    \end{minipage}
\end{figure*}



% $$DCG = \sum_{i=1}^{c} \frac{2^{rel(i)} - 1}{log_2(i+1)} $$ 

To account for the two-dimensional position bias, we define as $l$ the number of recommendation lists (\idest carousels) and extend the relevance function to two dimensions as $rel(i,j)$. The item relevance will be discounted by a quantity proportional to its position in both dimensions.
Thus, we define DCG2D as shown in Eq. \ref{eq:dcg2d}.
%Thus, we define DCG2D as:
% $$DCG2D = \sum_{i=1}^{l} \sum_{j=1}^{c}  \frac{2^{rel(i,j)} - 1}{log_2(i+j)}$$
% \mf{ok ma penso la prendessi un po' troppo alla larga}
% Let us assume a scenario where a model recommends a ranked list of $m$ items for a fixed user. We can assume that there is a ground truth of the relevance of items for the fixed user, given by $rel_i$ for the $i$\textsuperscript{th} item in the ranked list. In this scenario, we define the following accuracy metric, called \textit{Cumulative Gain} (CG), as $CG = \sum_{i=1}^{m} rel_i $. Still, this metric does not take into account the ranking of the items on the list. Hence, a variation of CG was proposed for this reason. This variation is the \textit{Discounted Cumulative Gain} (DCG), and it is defined as $DCG = \sum_{i=1}^{m} \frac{2^{rel_i} - 1}{log_2(i+1)} $. 
% To better evaluate the latter metric, it is mainly used in its normalized form, that is the \textit{Normalized Discounted Cumulative Gain} (nDCG), which is defined as $nDCG= DCG/IDCG$, where IDCG is the \textit{Ideal Discounted Cumulative gain}, defined as the DCG of the ideal ranked list, i.e. the list composed of the $m$ most relevant items, ranked with an ideal ranking according to the relevance of each item. 
% However, these metrics are not suitable for our two-dimensional scenario. In this case, the items recommended by a model will be in the form of a matrix. We call $r$ the number of rows to show to the user, and $c$ the number of items for each row (i.e., the columns of the matrix). Therefore, now the relevance will be given by $rel_{ij}$ for the item in position $(i,j)$. Also, we must redefine the previous metrics according to this new task. Here we make the assumption that the top-left corner of the matrix is the part where the user focuses more, and therefore is the most relevant one. In other words, we aim to define a metric where the item ranked in position $(i,j)$ will be discounted depending on the value of $i+j$. 
% Thus, we define DCG2D as 
% $$DCG2D = \sum_{i=1}^{r} \sum_{j=1}^{c}  \frac{2^{rel_{ij}} - 1}{log_2(i+j)}$$
This metric
%, assigns the same importance to all the slots on the same diagonal of the screen. 
allows to give importance to both dimensions, according to the weights ($\alpha, \beta \geq 1$) provided, which can vary depending on the use case. 
%For instance, a relevant item in row 1, column 3 has the same importance as a relevant item in row 3, column 1.
% \nico{r2 dice: The proposed 2D NDCG metric assigns the same importance to all the slots on the same diagonal of the screen. I think the metric should be flexible enough to enable the asymmetry of browsing rows and columns with different likelihoods.} \nico{RISOLTO: alpha, beta per la penalità}
%\nico{siamo sicuri di voler modificare la penalita'? perche' poi si potrebbe confondere con quella di SIGIR, che invece sembra un'estensione. Comunque si puo' fare con sforzo 0 perche' basta poi dire che negli esperimenti abbiamo preso alpha e beta uguali a 1.}
Accordingly, we define its normalized version as $NDCG2D = DCG2D/IDCG2D$. Similarly to NDCG, the IDCG2D will be the DCG2D of the \textit{ideal ranking}, which is the matrix composed of the user's %$r \cdot c$
%most relevant items, ranked according to the previously defined two-dimensional position discount, following constraint:$\forall (i,j), (h,k)$, $ rel(i,j) \geq rel(h,k)  $ if $ i+j < h+k $ .\nico{sistema} 
most relevant items, ranked according to the previously defined two-dimensional position discount, following constraint:
for any pair of cells $(i,j), (h,k)$ of the matrix,  $ rel(i,j) \geq rel(h,k)  $ if $ \alpha i+ \beta j < \alpha h+ \beta k $.
Notice how, in the case of different carousel lengths, the NDCG2D metric can be easily computed by assuming that all the carousels have the maximum carousel length and by treating the missing recommendations at the end of the shorter carousels as simply non-relevant.
% and the "holes" of the shorter carousels being non-relevant items.

% \nico{bozza: Notice how, in the case of different carousel lengths, the NDCG2D metric can be easily applied by assuming that all the carousels have the maximum carousel length and the holes being non-relevant items.}
% A comparison of the ranking discounts given by DCG and DCG2D can be found in Figure \ref{fig:dcg_vs_dcg2d_heatmap}.

% The assumption upon which the definition of this metric relies is motivated by many real-world examples, including the dataset released with \cite{DBLP:conf/cikm/MaureraDSSC20}.
% In this scenario, the phenomenon of decreasing attention from the top-left corner both to the right and to the bottom is evident from the visualization of the number of interactions shown in Fig. \ref{fig:cw_heatmap}. 
    



% \begin{figure*}[]
%     \centering
%     \begin{minipage}{0.4\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth]{images/contentwise_heatmap.pdf}
%         \caption{Heatmap of the number of interactions per position on the screen taken from
%         %the dataset presented in 
%         \cite{DBLP:conf/cikm/MaureraDSSC20}. 
%         %Values are log-scaled.
%         }
%         \label{fig:cw_heatmap}
%     \end{minipage}
%         \hfill
%     % \begin{minipage}{.49\textwidth}
%     %     \centering
%     %     \includegraphics[width=.98\textwidth]{images/ndcg2d_heatmap.pdf}
%     %     \caption{Heatmap of the weights given to each cell according to the DCG2D definition. The clearest cells are the ones that weigh the most (namely, the items in those cells should be the most relevant).\mf{rendere uniformi gli assi e inserire la scala di valori}}
%     %     \label{fig:dcg2d_heatmap}
%     % \end{minipage}%
%     \begin{minipage}{.45\textwidth}
%         % \centering
%         % \includegraphics[width=0.70\textwidth]{images/serp-google-golden-triangle-300x296.png}
%         % \caption{A known visualization of how users navigate a simple search result page, the attention is focused on a top-left \emph{golden triangle} and progressively decreases moving to the right and the bottom \cite{DBLP:conf/wsdm/ChierichettiKR11}.
%         % }
%         % \label{fig:ir_positionbias}
%         %\begin{table}
%         % \centering
%         % \small
%         % \begin{tabular}{|c|c|}
%         % \toprule
%         % Optimizing NDCG & Optimizing NDCG2D \\
%         % \midrule
%         % FunkSVD         &  FunkSVD      \\
%         % UserKNN         &  UserKNN      \\
%         % \textbf{IALS}   &  \textbf{NMF}          \\
%         % MF BPR          &  MF BPR       \\
%         % SLIM            &  SLIM         \\
%         % \textbf{NMF}    &  \textbf{IALS}         \\
        
%         % \bottomrule
%         % \end{tabular}
%         % \caption{Layouts obtained optimizing NDCG and NDCG2D.}
%         % \label{tab:results}
% %\end{table}

%             \centering
%         \small
%         \begin{tabular}{|c|c|}
%         \toprule
%         Optimizing NDCG & Optimizing NDCG2D \\
%         \midrule
%         SLIM EN         &  SLIM EN      \\
%         NMF         &  SLIM BPR      \\
%         \bottomrule
%         \end{tabular}
%         \caption{Layouts obtained optimizing NDCG and NDCG2D.}
%         \label{tab:results}

%     \end{minipage}%

% \end{figure*}


% \begin{figure*}[]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=1.1\textwidth]{images/heatmap_ndcg1d_log.pdf}
%         \caption{Heatmap of the weights given to each cell according to their position in the DCG definition. % The clearest cells are the ones that weigh the most (namely, the items in those cells should be the most relevant). Values are log-scaled.\mf{e se la facessi da bianco a blu?} \nico{come ti sembra ora?}
%         }
%         \label{fig:dcg_heatmap}
%     \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{.49\textwidth}
%         \centering
%         \includegraphics[width=1.1\textwidth]{images/heatmap_ndcg2d_log.pdf}
%         \caption{
%         Heatmap of the weights given to each cell according to their position in the DCG2D definition.% The clearest cells are the ones that weigh the most (namely, the items in those cells should be the most relevant). Values are log-scaled.
%         % \mf{rendere uniformi gli assi e inserire la scala di valori}
%         }
%         \label{fig:dcg2d_heatmap}
%     \end{subfigure}%
% \caption{
%     Heatmap of the weights attributed to each cell based on its position. Figure \ref{fig:dcg_heatmap} represents the DCG metric where the user is assumed to explore the carousels sequentially, while Figure \ref{fig:dcg2d_heatmap} represents our proposed extension DCG2D. Darker cells indicate lower weight, values are log-scaled. We can see how the proposed DCG2D mirrors more closely the user behavior by attributing higher weight to the top-left corner. \nico{r2 dice che questa figura non aggiunge molto al discorso}
%     }   
%     \label{fig:dcg_vs_dcg2d_heatmap}
% \end{figure*}


% \subsubsection{Accuracy metrics:} Each correct recommendation is considered only once.
% \subsubsection{Ranking metrics:} Each correct recommendation is considered only once and is associated to the position of the first occurrence in the recommendation list. Subsequent occurrences of the same item are ignored but not removed from the recommendation list in order to maintain unaltered the positions of other relevant recommendations.

% \subsubsection{Beyond-accuracy metrics:} \nico{forse da togliere} Another important dimension to be taken into account when evaluating recommendation models is their diversity. In a carousel evaluation setting the metrics used for the traditional top-n recommendation scenario can be used seamlessly simply providing the recommendations of all carousels concatenated in a single recommendation list. 
% %The items appearing in multiple carousels should not be removed.
% In this setting it will be possible to calculate correctly several commonly used beyond-accuracy metrics: Item Coverage (the quota of items that have been recommended at least once), Average Popularity (the average popularity of the recommended items), Novelty (mean self-information \cite{zhou2010solving}, a function of the item popularity in the train data). The same applies for \emph{distributional diversity} metrics, computed on the global number of times each item has been recommended, the more unbalanced the distribution is, the less diverse the model is: Shannon diversity, Gini diversity and Herfindahl Index \cite{DBLP:journals/tkde/AdomaviciusK12,FerraridacremaDemonstrating2021}.
% A notable exception is \emph{Mean inter-list diversity} (MIL) \cite{zhou2010solving}, which measures the average number of recommended items each couple of users has in common. The formulation is not well-defined in case duplicate items appear, moreover removing them would produce erroneous results since MIL is defined as an arithmetic mean and requires recommendation lists of the same length. We can also mention that a recently published proof in  \cite{FerraridacremaDemonstrating2021} shows that MIL is equivalent to the Herfindahl Index under the traditional top-n recommendation setting is based on the implicit assumption that the recommendations do not contain duplicates, hence, this equivalence does not hold in a carousel setting.








% How to consider duplicate items depends on the specific metric:
% \begin{description}
%     \item[Item Coverage:] The metric computes the quota of items that have been recommended at least once. It is unaffected by duplicates since it is not sensitive to the number of times the item has been recommended;
%     \item[Average Popularity:] The metric computes the average popularity of the items in each user's recommendation list and is then averaged across all users. Being an arithmetic mean it requires all users have the same recommendation list length. It is reasonable to retain duplicated items as they contribute to the average popularity of the overall recommendation list.
%     \item[Novelty:] The metric is the mean self-information \mf{citation} and is a function of the item popularity in the train data, the less popular an item is the more novel a recommendation is. Duplicates not removed.
%     % In this case, a duplicate item would not contribute anything to the novelty of the recommendation list and therefore can be considered having novelty of zero. Since this metric is cumulative on all recommendations, duplicated items should be removed from the user's recommendation list. \mf{verificare se vi piace}
%     \item[Distributional Diversity:] diversity metrics such as Shannon Gini and Herfindahl are based on the number of times each item has been recommended. The presence of duplicated items would not improve the diversity of the recommendations, hence duplicated items should be removed.
%     \item[List-based diversity: ] \mf{RIFARE}metrics such as Mean Inter-List diversity measure the average quota of the recommendation list any two users have in common. The presence of duplicated items would increase this quota and reduce the overall diversity. Furthermore, recently Ferrari Dacrema \mf{cit} demonstrated this metric is equivalent to the distributional diversity Herfindahl index. This equivalence however only holds under the assumption that the recommendation list contains no duplicates. If duplicates are present, the inter-list similarity between users becomes asymmetric and the equivalence does not hold anymore. \mf{attenzione. Se due utenti hanno un item in comune, ma l'utente A lo ha duplicato, il numero di item in comune tra loro è calcolato come 2. La diversity di A->B è corretta ma quella di B->A no. Se hanno un item in comune ed in entrambi è duplicato il count diventa 4, se non fosse stato duplicato sarebbe 5. La progressione è combinatoria. Da valutare con attenzione} Developing a new formulation of MIL applicable in this scenario is a future work. \mf{forse si può salvare se nelle occorrenze degli item metto solo i non duplicati, ma poi si romperebbe la lunghezza delle liste}
% \end{description}


\section{Experimental Analysis}
\label{sec:experimental_anaysys}
%\nico{dire che vogliamo evidenziare common trends e differenze nei due scenari di valutazione.}
In this section we apply the proposed carousel evaluation on 
%numerous 
widely used algorithms and compare the results obtained with the traditional evaluation which considers each model independently. We discuss the results of this comparison and highlight some common trends and differences. We release the source code for our experiments in an online repository.\footnote{\url{https://github.com/nicolo-felicioni/RecSysCarouselEvaluation}}

\subsection{Algorithms} 
In our evaluation, we included several algorithms developed in the last three decades of research, trying to obtain a broad picture of different families of models.
%. We tried to obtain a picture that is as broad as possible, including algorithms from different families in our measurements. %An overview of the algorithms used is in Table \nico{todo}. \nico{where to put the hyperparameters?} 
%We did not include more complex neural models due to their limited reproducibility and significant computational cost \cite{10.1145/3434185}, we leave this as a future work.

\begin{itemize}
    \item \emph{Non-Personalized.} A simple but effective 
    % non-personalized
    model, \textbf{TopPopular} recommends to all users the most popular items. 
 
    \item \emph{Nearest-Neighbor Methods.} 
    We include in our analysis collaborative filtering (CF) nearest-neighbor techniques %\cite{DBLP:conf/cscw/ResnickISBR94}
    such as \textbf{ItemKNN} %\cite{sarwar2001item}
    , based on item-item similarities and \textbf{UserKNN} %\cite{DBLP:conf/www/SarwarKKR01}
    based on user-user similarities. In both cases the similarity is computed with cosine similarity with shrinkage.% \cite{bell2007improved}. 
    
    \item \emph{Graph-based Methods.} 
    We select two simple approaches that model a random walk in a graph containing user and item nodes.
    In \palphabold \cite{DBLP:conf/www/CooperLRS14} the similarity between items is computed as the transition probability between them. 
    \pbetabold  \cite{DBLP:journals/tiis/PaudelCNB17} extends \palpha dividing the similarity between two items by their popularity, raised to the power of an additional hyperparameter $\beta$, in order to reduce the popularity bias of the algorithm.

    \item \emph{Content-based and Hybrid Methods.} To account for content information we also include content-based models. Among the simplest content based models are neighborhood-based methods that build item-item similarities based on features, \textbf{ItemKNN-CBF} computes the item-based similarity using the item features while \textbf{UserKNN-CBF} computes the user-based similarity using user features. We use the cosine similarity with shrinkage.
    These methods can be easily extended by creating a new feature vector which concatenates both collaborative and content data %\cite{DBLP:conf/ewmf/MobasherJZ03}
    . The resulting hybrid algorithms are \textbf{ItemKNN-CFCBF} and \textbf{UserKNN-CFCBF}.
    
    \item \emph{Machine Learning Approaches.} We include several simple but well-known models relying on machine learning, like \textbf{SLIM ElasticNet (EN)} \cite{levy2013SLIM_ElasticNet}, a scalable variant of the original SLIM% \cite{ning2011SLIM}
    , and \textbf{SLIM BPR}, a variant of SLIM minimizing the BPR loss. % \cite{DBLP:conf/uai/RendleFGS09}.
    We also include a recent method called \textbf{\EASER} \cite{DBLP:conf/www/Steck19}, where the author showed how an "embarrassingly shallow" linear model with closed-form solution can outperform much more complex techniques. 
    
    \item \emph{Matrix Factorization Techniques.} We include various matrix factorization algorithms, like \textbf{PureSVD} \cite{DBLP:conf/recsys/CremonesiKT10}, \textbf{FunkSVD}%\footnote{\url{https://sifter.org/~simon/journal/20061211.html}}
    , which are developed for explicit ratings, and \textbf{iALS} %\cite{DBLP:conf/icdm/HuKV08}
    , \textbf{Non-negative Matrix Factorization (NMF)} %\cite{DBLP:journals/ieicet/CichockiP09}
    , \textbf{Matrix Factorization (MF) BPR} %\cite{DBLP:conf/uai/RendleFGS09}
    , focusing on implicit feedback.

\end{itemize}



% ============= % ============= % ============= BEGIN ALGORITHM LIST ============== ============== ============== ============== ==============

% \paragraph{Popularity-based.} A simple but effective non-personalized model, \textbf{TopPopular} recommends to all users the most popular items. 
% % \paragraph{Top-Popular.}
% % The TopPopular is a popularity-based non-personalized ranking algorithm. It recommends to every user the most popular items. The popularity of an item is calculated by counting the number of its (implicit or explicit) ratings. 

% \paragraph{Nearest-Neighbor Methods.} 
% % \paragraph{ItemKNN-CF}
% We include in our analysis collaborative filtering (CF) nearest-neighbor techniques \cite{DBLP:conf/cscw/ResnickISBR94} such as \textbf{ItemKNN} \cite{sarwar2001item}, based on item-item similarities and \textbf{UserKNN} \cite{DBLP:conf/www/SarwarKKR01} based on user-user similarities. In both cases the similarity is computed with cosine similarity with shrinkage \cite{bell2007improved}. 
% % Nearest-neighbor techniques are simple and widely adopted methods that were first used in the early GroupLens system \cite{DBLP:conf/cscw/ResnickISBR94}. As collaborative filtering (CF) algorithms we include in our analysis both \textbf{ItemKNN} \cite{sarwar2001item}, based on item-item similarities and \textbf{UserKNN} \cite{DBLP:conf/www/SarwarKKR01} based on user-user similarities. In both cases the similarity is computed with cosine similarity with shrinkage \cite{bell2007improved}. 
% % For the ItemKNN the similarity is computed as follows: % including shrinkageThis variant builds item-item similarities to make recommendations. In this research, we used the cosine similarity, defined as 
% % $$ s_{ij} = \frac{\textbf{r}_i \cdot \textbf{r}_j}{|| \textbf{r}_i || \ || \textbf{r}_j || + h}$$
% % where $\textbf{r}_i, \textbf{r}_j \in \mathbb{R}^{|U|}$ are the vectors containing the (implicit or explicit) interactions of each user for items $i$ and $j$, respectively, and $|U|$ is the number of users in the dataset. The shrink term $h$ is needed to lower the similarity of items having few ratings \cite{bell2007improved}.
% % While nearest-neighbor methods only consider the common items or users, graph-based models allow a broader representation of neighborhood.
% We also select two simple approaches that model a random walk in a graph containing user and item nodes.
% %, two nodes are connected if there is an interaction between them. 
% In \palphabold \cite{DBLP:conf/www/CooperLRS14} the similarity between items is computed as the transition probability between them. 
% %Graph-based algorithms aim to improve traditional nearest-neighbor approaches relying on a broader interpretation of neighborhoods. Indeed, this method implements a two-steps random walk from users to items and vice-versa \cite{DBLP:conf/www/CooperLRS14}. In order to implement a random walk, each user-item jump must have a probability assigned. 
% %This probability is computed from the normalized ratings raised to the power of $\alpha$. 
% % In the original paper it is stated that, \palpha is equivalent to an ItemKNN algorithm, where the similarity matrix is computed as the dot-product of the probability vectors. In addition, we select the k most similar items and normalize each row of the similarity matrix with its $\ell_1$ norm to ensure they represent a probability distribution, as done in \cite{10.1145/3434185}. The hyperparameters of the algorithm include the neighborhood size and the value of $\alpha$.
% \pbetabold  \cite{DBLP:journals/tiis/PaudelCNB17} is an extension of \palpha, where the similarity between two items is 
% %computed with \palpha and then
% divided by the popularity of the two items raised to the power of an additional hyperparameter $\beta$, in order to reduce the popularity bias of the algorithm.
% % Again, we normalize each row of the similarity matrix with its $\ell_1$ norm.
% % Notice that if the value of $\beta$ is 0, \pbeta is equivalent to \palpha. The hyperparameters include $\alpha$, $\beta$, and the neighborhood size.


% % \paragraph{UserKNN-CF}
% % A neighborhood-based technique that builds user-user similarities in a collaborative way. Hyperparameters are the same as used for ItemKNN-CF \cite{DBLP:conf/www/SarwarKKR01}.

 
% % \paragraph{Graph-based Methods.} 
% % While nearest-neighbor methods only consider the common items or users, graph-based models allow a broader representation of neighborhood.
% % We select two simple approaches that model a two-steps random walk in a bipartite graph containing user and item nodes.
% %, two nodes are connected if there is an interaction between them. 
% % In \palphabold \cite{DBLP:conf/www/CooperLRS14} the similarity between items is computed as the transition probability between them. 
% %Graph-based algorithms aim to improve traditional nearest-neighbor approaches relying on a broader interpretation of neighborhoods. Indeed, this method implements a two-steps random walk from users to items and vice-versa \cite{DBLP:conf/www/CooperLRS14}. In order to implement a random walk, each user-item jump must have a probability assigned. 
% %This probability is computed from the normalized ratings raised to the power of $\alpha$. 
% % In the original paper it is stated that, \palpha is equivalent to an ItemKNN algorithm, where the similarity matrix is computed as the dot-product of the probability vectors. In addition, we select the k most similar items and normalize each row of the similarity matrix with its $\ell_1$ norm to ensure they represent a probability distribution, as done in \cite{10.1145/3434185}. The hyperparameters of the algorithm include the neighborhood size and the value of $\alpha$.
% % \pbetabold  \cite{DBLP:journals/tiis/PaudelCNB17} is an extension of \palpha, where the similarity between two items is 
% %computed with \palpha and then
% % divided by the popularity of the two items raised to the power of an additional hyperparameter $\beta$, in order to reduce the popularity bias of the algorithm.
% % Again, we normalize each row of the similarity matrix with its $\ell_1$ norm.
% % Notice that if the value of $\beta$ is 0, \pbeta is equivalent to \palpha. The hyperparameters include $\alpha$, $\beta$, and the neighborhood size.




% \paragraph{Content-based and Hybrid Methods.} To account for content information we also include some simple content-based models. Among the simplest content based models are neighborhood-based methods that build item-item similarities based on features, \textbf{ItemKNN-CBF} computes the item-based similarity using the item features while \textbf{UserKNN-CBF} computes the user-based similarity using user features. In this case as well we use the cosine similarity with shrinkage.
% These methods can be easily extended by creating a new feature vector which concatenates both collaborative and content data \cite{DBLP:conf/ewmf/MobasherJZ03}. The resulting hybrid algorithms are \textbf{ItemKNN-CFCBF} and \textbf{UserKNN-CFCBF}.

% % \paragraph{Content-based} Among the simplest content based models are neighborhood-based methods that build item-item similarities based on features, \textbf{ItemKNN-CBF} computes the item-based similarity using the item features while \textbf{UserKNN-CBF} computes the user-based similarity using user features. In this case as well we use the cosine similarity with shrinkage.

% % In case of ItemKNN-CBF the similarity computed will be:
% % $$ s_{ij} = \frac{\textbf{f}_i \cdot \textbf{f}_j}{|| \textbf{f}_i || \ || \textbf{f}_j || + h}$$
% % where $\textbf{f}_i, \textbf{f}_j \in \mathbb{R}^{|F|}$ are the vectors containing the feature values for items $i$ and $j$, respectively and $|F|$ is the number of features.
% % The hyperparameters are the same as for the collaborative filtering techniques \cite{DBLP:reference/rsh/LopsGS11}.

% % \paragraph{UserKNN-CBF}
% % Similar to the ItemKNN-CBF, but it aims to build user-user similarities (instead of item-item ones) using user's content features (instead of items' ones).

% % \paragraph{Hybrid Methods}
% % A simple neighborhood-based hybrid can be built by creating a new feature vector which concatenates both collaborative and content data \cite{DBLP:conf/ewmf/MobasherJZ03}. In \textbf{ItemKNN-CFCBF} the vector of the item ratings (collaborative features) is concatenated with the vector of the item attributes (content features). In \textbf{UserKNN-CFCBF} the same principle applies by concatenating the user profile vector with the user feature vector.
% % Then, the item-item or user-user similarities will be computed with a cosine similarity with shrinkage.
% % The hyperparameters are the same as for the collaborative filtering algorithms. A new hyperparameter $w$ regulates the relative weight of the content features with respect to the collaborative ones. If $w$ is 0, this algorithm is equivalent to the ItemKNN-CF.

% % \paragraph{UserKNN-CFCBF}
% % This algorithm is almost the same as ItemKNN-CFCBF, but it aims to build user-user similarities. Therefore, in this version, the users' implicit rating vectors and the users' attribute vectors will be concatenated and used to build the similarities.

% \paragraph{Machine Learning Approaches.} In this analysis we also include several simple but well-known models relying on machine learning, like \textbf{SLIM EN} \cite{levy2013SLIM_ElasticNet}, a scalable variant of the original SLIM \cite{ning2011SLIM},
% and \textbf{SLIM BPR}, a variant of SLIM minimizing the BPR loss \cite{DBLP:conf/uai/RendleFGS09}. Also, we included a recent method called \textbf{\EASER} \cite{DBLP:conf/www/Steck19}, where the author showed how an "embarrassingly shallow" linear model with closed-form solution can outperform much more complex techniques proposed in the literature. 

% \paragraph{Matrix Factorization Techniques.} We include various matrix factorization algorithms, like \textbf{PureSVD} \cite{DBLP:conf/recsys/CremonesiKT10}, \textbf{FunkSVD}\footnote{\url{https://sifter.org/~simon/journal/20061211.html}}, which are developed for explicit ratings, and \textbf{iALS} \cite{DBLP:conf/icdm/HuKV08}, \textbf{Non-negative Matrix Factorization (NMF)} \cite{DBLP:journals/ieicet/CichockiP09}, \textbf{Matrix Factorization (MF) BPR} \cite{DBLP:conf/uai/RendleFGS09}, focusing on implicit feedback.

% ============= % ============= % ============= END ALGORITHM LIST ============== ============== ============== ============== ==============




% \paragraph{Matrix Factorization (MF) Techniques}
% This techniques trace their roots into the early years of recommender systems \cite{DBLP:conf/icml/BillsusP98}. In fact, they became a de-facto standard after they gained popularity during the Netflix prize competition (2006-2009). In this research, we examined four different MF variants:

% \begin{itemize}
%     \item \textbf{iALS.} 
%     This algorithm was proposed in \cite{DBLP:conf/icdm/HuKV08}, where the authors presented an Alternating Least Squares approach focusing exclusively on implicit feedback datasets. 
%     %The core of this method is the formulation of confidence values starting from implicit feedback. 
%     % There are several hyperparameters that can be tuned for this method, like the number of latent factors, the confidence scaling, and the regularization factor.
    
%     \item \textbf{PureSVD.}
%     This method was proposed by \cite{DBLP:conf/recsys/CremonesiKT10} and relies on the SVD decomposition of the interaction data. We use a standard decomposition from the \texttt{scikit-learn} Python package.
%     % The only hyperparameter is the number of latent factors.
%     \item \textbf{FunkSVD.}
%     This method was described by Simon Funk in its well known online article\footnote{\url{https://sifter.org/~simon/journal/20061211.html}} during the Netflix Prize. It optimizes explicit rating prediction minimising the mean squared error. 
%     % In order to use FunkSVD for top-n recommendation problems, a hyperparameter can be added to ensure a certain number of training samples are randomly sampled among the unseen items, associating them with a rating of 0, as done in \cite{10.1145/3434185}. There is a hyperparameter to decide if the model should include global bias, user bias, or item bias. Other hyperparameters are the learning rate, the regularization coefficients for the Frobenius norm, and the number of latent factors.
    
%     \item \textbf{Non-negative Matrix Factorization (NMF).} This method is described in \cite{DBLP:journals/ieicet/CichockiP09}. Unlike PureSVD, this method ensures that all latent factors are positive. Our implementation relies on the standard NMF decomposition provided in the \texttt{scikit-learn} package for Python.\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.decomposition.NMF.html}} 
%     % The only hyperparameter is the number of latent factors.
    
%     \item \textbf{Matrix Factorization (MF) BPR.} This algorithm was introduced in \cite{DBLP:conf/uai/RendleFGS09} and optimizes the \textit{Bayesian Personalized Ranking} (BPR) loss. The loss was designed to maximize ranking accuracy rather than rating prediction. %Indeed, MF BPR was explicitly designed for implicit feedback datasets, differently from PureSVD, FunkSVD, and NMF. 
%     % The hyperparameters are the number of latent factors, the learning rate, and the regularization coefficients.
    
    
% % \end{itemize}


% % \paragraph{Sparse Linear Models (SLIM)}
% % SLIM was proposed in \cite{DBLP:conf/icdm/NingK11}. It is a well-performing regression-based method for top-n recommendation tasks. In our research, we use two variants:
% % \begin{itemize}
%     \item \textbf{SLIM EN.}
%     It is a scalable variant of the original SLIM \cite{ning2011SLIM}, proposed in \cite{levy2013SLIM_ElasticNet},
%     learning the item similarity matrix one item at a time (i.e., one column at a time). 
%     % This is done by solving a regression problem which learns the interactions for the target item by using the interactions of all the other items available in the training data. 
%     Our implementation relies on the standard EN solver provided in the \texttt{scikit-learn} Python package.
    
%     \item \textbf{SLIM BPR.} 
%     This algorithm is a variant of SLIM which learns an item-item similarity matrix minimizing the BPR loss \cite{DBLP:conf/uai/RendleFGS09}. Therefore, it aims to maximize ranking accuracy rather than optimizing rating prediction \cite{DBLP:conf/um/AnelliBNBTS17, DBLP:conf/sigir/BalogRA19, DBLP:conf/um/Suglia0MGLS17}. 
%     % The hyperparameters include the number of neighbors, the regularization coefficients, and a boolean flag that indicates whether the similarity matrix should be symmetric or not.


%     \item \textbf{\EASER.}
% This method was proposed recently in \cite{DBLP:conf/www/Steck19}, where the author showed how an "embarrassingly shallow" linear model can outperform much more complex techniques proposed in the literature. The algorithm is based on an auto-encoder, but there exists a closed-form solution which results in very fast training.
% \end{itemize} 



\subsection{Hyperparameter optimization} 
While in this paper we do not aim to show that any particular model is superior to others, we nonetheless ensure that all algorithms are 
% fairly and 
consistently optimized. To do so we followed the best practices highlighted by \citet{10.1145/3434185} and we relied on the framework published, using a Bayesian search \cite{DBLP:conf/recsys/FelicioniDCBHBD20} %, DBLP:conf/recsys/AntenucciBCDKSD18}
%\footnote{The framework implementation relies on the Scikit-optimize package \url{https://scikit-optimize.github.io/}}
optimizing the MAP metric at cutoff 10.
% We searched the optimal hyperparameters for each model and for each dataset with a Bayesian search \cite{DBLP:conf/recsys/FelicioniDCBHBD20, DBLP:conf/recsys/AntenucciBCDKSD18}\footnote{The framework implementation relies on the Scikit-optimize package \url{https://scikit-optimize.github.io/}} optimizing the recommendation quality on a validation split, measured with MAP at cutoff 10. We explored 50 cases for each algorithm, the first 15 used as random initialization. Once the optimal hyperparameters were found, the final model was fitted on the union of the training and validation data and was evaluated on the test data. The hyperparameter ranges and distribution used during the optimization are the same used and reported in \cite{10.1145/3434185}.

\subsection{Datasets}
% We report the results for some widely known and used datasets, all of which are publicly available.
We report the results for some widely used  publicly available datasets.
We only selected datasets from domains that tend to use the carousel user interface, in particular video-on-demand. 
We included \textit{MovieLens 10M}, %\cite{DBLP:journals/tiis/HarperK16}
, a popular dataset of movies recommendations, with 69,878 users, 10,681 items and 10M ratings. The dataset contains user provided tags for items as well as the year of release and the genre.
%and music streaming
%In this section we list the datasets we selected and the preprocessing applied, statistics of the datasets after preprocessing are reported in Table \ref{tab:datasets}.
% Statistics of the datasets after preprocessing are reported in Table \ref{tab:datasets}.
We conducted experiments also on the \textit{Netflix} dataset %\cite{bennett2007netflix}
, which is the well known movie dataset from the \textit{Netflix Prize}. To reduce the computational time, we randomly sampled 20\% of the users. After pre-processing, this dataset has 95,965 users, 17,768 items and almost 20M ratings. 
After pre-processing, we randomly selected 80\% of interactions for the training set and 10\% for both validation and test set.


% \begin{table}[]
% \centering
% \small
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Dataset       & Users &         Items & Ratings &   Density & Gini index \\ \hline \hline
% % MovieLens 1M  &   6,048    &    3,883   &  \textasciitilde 1M       &  4.26 \%     &  0.53 \\ \nico{not necessary anymore}
% MovieLens 10M &    69,878   &   10,681    &     \textasciitilde 10M    & 1.34 \%    &  0.57 \\
% %Spotify       & 89,851      &   71,849    &     \textasciitilde 5M   &    0.08 \%   & 0.41  \\
% Netflix       &   95,965     &   17,768    &    \textasciitilde 20M    &    1.17 \%   & 0.60 \\ \hline
% \end{tabular}
% \caption{Overview of the datasets after preprocessing.\nico{si può inserire nel testo}}
% \label{tab:datasets}
% \end{table}



% \begin{itemize}
%     % \item \textit{MovieLens 1M}\footnote{\url{https://grouplens.org/datasets/movielens/1m/}} \mf{forse da togliere se non ne parliamo} \cite{DBLP:journals/tiis/HarperK16}. %, a very popular dataset taken from a movie recommendation website maintained by the \textit{GroupLens} research group, from the University of Minnesota. 
%     % It contains approximately 1M explicit ratings going from 1 to 5, with 6,048 users and 3,883 items. Besides, the dataset contains content features regarding users and items. 
%     % User information provided includes gender, age, and occupation. Regarding the items, we are provided with the titles of the movies and their genres. In our experiments, we used only the genre content information.
%     \item \textit{MovieLens 10M}
%     %\footnote{\url{https://grouplens.org/datasets/movielens/10m/}} 
%     \cite{DBLP:journals/tiis/HarperK16}, a very popular dataset of movies recommendations. %, composed of approximately 10M ratings, with 69,878 users and 10,681 items. In dataset there is no user information provided, but there are the titles of the movies. 
%     The dataset contains user provided tags for items as well as the year of release and the genre. %In our experiments, we used genre and year.
%     % \item \textit{Spotify}\footnote{\url{https://www.aicrowd.com/challenges/spotify-million-playlist-dataset-challenge}} \cite{DBLP:conf/recsys/ChenLSZ18}, was released as \textit{Million Playlists Dataset} for the \textit{RecSys Challenge 2018}. In this dataset the items are songs and the users are represented by user created playlists. %, contains one million user-created playlists, for a total amount of approximately 2 millions unique tracks. 
%     %  %The playlists were created during the period of early 2010 until late 2017.
%     % %The objective of the challenge was playlist continuation, i.e., creating a model that, for each playlist, suggests tracks to add to the playlist. In this scenario, we consider the playlists as the users, while the tracks are the items. 
%     % Due to the big size of the dataset, to reduce the computational time we randomly sampled 10\% of the playlists and then ensured both users and items have at least 10 interactions. The resulting dataset is denser than the original one but still the sparsest of those we report. %, and then \nico{TODO i don't know what it is but we applied DataPostprocessing\_K\_Cores(k\_cores\_value=10).}
%     % % For each playlist, content features provided include the title of the playlist, the list of tracks, the number of followers, and others. \nico{which are the items? playlists or tracks?}
%     \item \textit{Netflix}
%     %\footnote{\url{https://www.kaggle.com/netflix-inc/netflix-prize-data}}
%     \cite{bennett2007netflix}, is the well known movie dataset from the \textit{Netflix Prize}. %The original dataset contains over 100 million ratings from 480,189 users. % n of ratings: 100480507
%     %In total, there are 17,770 movies in the dataset. The ratings were collected during the period of late 1998 until late 2005. The ratings are explicit, on a scale from 1 to 5. 
%     To reduce the computational time, we randomly sampled 20\% of the users.
% \end{itemize}

% The statistical properties of the datasets after pre-processing are summarized in Table \ref{tab:datasets}.

% \subsection{MovieLens 1M}

% % KendalltauResult(correlation=0.6339869281045752, pvalue=0.00010483725733996005)

% \nico{Elenco di cose da dire:
%     -- Indagare se c'è una qualche proprietà speciale propria dei metodi matrix factorization, dato che SEMBRA che salgano nel ranking carousel.
%     -- Forse dovremmo dire qualcosa anche sui risultati NDCG2D, altrimenti la sua definizione potrebbe sembrare inutile.
% }

% Tables \ref{tab:ml1macc} and \ref{tab:ml1mbeyondacc} describe the performance of the various algorithms on the MovieLens 1M dataset, according to accuracy and beyond accuracy metrics, respectively. 

% For each metric, the tables show the performance with the standard Individual evaluation and the novel carousel evaluation. 

% Several considerations can be made looking at these results. 
% For instance, looking at the $\Delta_{TopPop}$ MAP column, we can notice how a standard Individual evaluation could be non-realistic in a carousel scenario. Indeed, if we take the ItemKNN CBF, we can see how this algorithm seemed to have much lower performance (MAP) with respect to the simple TopPop. Instead, if a carousel evaluation approach is adopted, it overperforms the TopPop by 13.34\%. This happens because of the different natures of the TopPop, which takes in input solely items popularities, and the ItemKNN CBF, which exploits only content information in order to make recommendations. In a scenario where the TopPop carousel is fixed as the top carousel due to business constraints, such a different point of view translates to an improvement of the user experience. This improvement could not be foreseen with the standard evaluation mode.
% Apart from the single example, we can notice a general trend from these data: the $\Delta_{TopPop}$ MAP presents always differences in the two evaluation modalities. 
% Hence, we believe that our evaluation procedure is necessary for real scenarios with carousels that we described before since it sheds light on hidden interactions among carousels that could not be visible with a standard evaluation approach.

% As further evidence of this, let us consider the situation where the provider of a streaming service homepage formed of carousels, with a fixed TopPop carousel on the top of the page, has to choose which algorithm's carousel present to the users. To do so, one could naively select the best performing algorithm according to some metric (let us assume it is MAP) with the standard Individual evaluation. As it can be seen from the Individual MAP rank column of Table \ref{tab:ml1macc}, the best MAP evaluated independently is provided by SLIM EN. This is not consistent, though, with our carousel evaluation protocol, where the same algorithm is 4\textsuperscript{th}. In fact, considering also the interactions among carousels, it can be observed how IALS is the best choice for the streaming service provider. 
% In general, looking at the difference between the rankings in the two evaluation protocols shown in the $\Delta$ MAP rank column, we can notice how many algorithms have different positions in the global ranking. Particularly relevant is the example of NMF, which from 13\textsuperscript{th} place reaches the 3\textsuperscript{rd} one. A proof of the difference between the two rankings is the fact that Kendall's $\tau$ coefficient of those is 0.634. This suggests that the two rankings are somehow correlated (as expected), but the fact that $\tau$ < 1 means that the Individual ranking is not sufficient to make any conclusion about the carousel MAP ranking. Therefore, this is another proof of the necessity of a novel evaluation protocol.  A visualization of the major differences between the two rankings is provided in Fig. \ref{fig:ml1m_ranking}.

% Given these results, we tried to analyze them in order to understand which could be the effect of the interaction among carousels. 
% In Fig. \ref{fig:ml1m_plots} and \ref{fig:ml1m_ndcg_plots}, we show some scatter plots of how MAP and NDCG metrics vary with respect to a beyond accuracy metrics. In particular, we selected the MIL diversity and the Novelty metrics. Due to their poor performance with both evaluation modes, we decided to exclude from the plot the purely content-based, the Random and the TopPop algorithms. \nico{non so se va bene come spiegazione} MAP and NDCG are evaluated following both the standard independent evaluation and the carousel evaluation protocol. For the NDCG, the carousel evaluation is done using our two-dimensional variant. For each of those plots, the trend line is shown as a red dashed line. Such a trend line is computed as the least-squares polynomial fit of the various points on the plot. The implementation used is NumPy \texttt{polyfit} function\footnote{\url{https://numpy.org/doc/stable/reference/generated/numpy.polyfit.html}}. The degree of the polynomial is two.
% Looking at those plots, it becomes clear how the beyond accuracy metrics are positively correlated with the carousel accuracy, while there was little to no correlation with the accuracy evaluated independently. 
% This result is noteworthy because it shows how, in a real scenario with carousels, the choice of which recommendation lists display should take into account how those lists complement each other. Therefore, lists that provide diversity or novelty may be beneficial when a TopPop carousel is fixed above them, given the alternative perspective they bring. Also, this provides another evidence of how popularity biased algorithms may harm the user experience in real scenarios \cite{DBLP:conf/recsys/AbdollahpouriMB19}. Furthermore, this result is consistent with previous observations on how a set of diverse and novel recommendations may improve user satisfaction \cite{chen2018fast, DBLP:conf/recsys/ZhangH08}. 

% \nico{An indication that the carousel evaluation protocol produces results consistent with previous observations in A/B testing \mf{diversity is better, cit. Verificare}}



% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &          Individual &           Carousel & Individual & Carousel &              {} \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D & \multicolumn{2}{c|}{$ \Delta_{TopPop} $ MAP} &       \multicolumn{2}{c|}{MAP rank} & $ \Delta $ rank \\
% \midrule
% TopPop          &         0.1057 & 0.0656 & 0.0879 &        0.0529 & 0.0426 & 0.0879 &  0.0849 &                  0.00\% &                  0.00\% &             16 &            18 &              -2 \\
% \midrule
% UserKNN CF      &         0.2240 & 0.1752 & 0.2253 &        0.1268 & 0.0674 & 0.1615 &  0.2033 &               +167.08\% &                +58.29\% &              5 &             9 &              -4 \\
% ItemKNN CF      &         0.2153 & 0.1668 & 0.2046 &        0.1255 & 0.0674 & 0.1550 &  0.1939 &               +154.31\% &                +58.25\% &             10 &            10 &               0 \\
% P3alpha         &         0.2142 & 0.1651 & 0.2080 &        0.1238 & 0.0664 & 0.1537 &  0.1910 &               +151.77\% &                +55.83\% &             11 &            11 &               0 \\
% RP3beta         &         0.2182 & 0.1686 & 0.2154 &        0.1264 & 0.0678 & 0.1586 &  0.1997 &               +157.09\% &                +59.15\% &              6 &             8 &              -2 \\
% \midrule
% \EASER          &         0.2360 & 0.1857 & 0.2325 &        0.1337 & 0.0702 & 0.1641 &  0.2079 &               +183.05\% &                +64.85\% &              2 &             5 &              -3 \\
% SLIM BPR        &         0.2121 & 0.1628 & 0.2206 &        0.1164 & 0.0638 & 0.1560 &  0.1935 &               +148.15\% &                +49.75\% &             12 &            13 &              -1 \\
% SLIM EN &         0.2477 & 0.1988 & 0.2475 &        0.1416 & 0.0740 & 0.1729 &  0.2230 &               +203.14\% &                +73.61\% &              1 &             4 &              -3 \\
% \midrule
% MF BPR          &         0.1865 & 0.1360 & 0.1690 &        0.1111 & 0.0616 & 0.1391 &  0.1671 &               +107.35\% &                +44.53\% &             14 &            14 &               0 \\
% MF FunkSVD      &         0.2198 & 0.1679 & 0.2147 &        0.1303 & 0.0693 & 0.1617 &  0.2037 &               +156.05\% &                +62.75\% &              8 &             6 &              +2 \\
% PureSVD         &         0.2292 & 0.1772 & 0.2234 &        0.1425 & 0.0753 & 0.1691 &  0.2168 &               +170.13\% &                +76.87\% &              4 &             2 &              +2 \\
% NMF             &         0.2109 & 0.1549 & 0.1930 &        0.1394 & 0.0741 & 0.1638 &  0.2063 &               +136.22\% &                +73.93\% &             13 &             3 &             +10 \\
% IALS            &         0.2392 & 0.1847 & 0.2177 &        0.1496 & 0.0788 & 0.1694 &  0.2156 &               +181.58\% &                +84.87\% &              3 &             1 &              +2 \\
% \midrule
% ItemKNN CBF     &         0.0495 & 0.0244 & 0.0315 &        0.0723 & 0.0483 & 0.0994 &  0.1025 &                -62.84\% &                +13.34\% &             17 &            15 &              +2 \\
% UserKNN CBF     &         0.1117 & 0.0705 & 0.0980 &        0.0665 & 0.0463 & 0.1003 &  0.1052 &                 +7.51\% &                 +8.60\% &             15 &            16 &              -1 \\
% ItemKNN CFCBF   &         0.2159 & 0.1668 & 0.2063 &        0.1265 & 0.0678 & 0.1570 &  0.1969 &               +154.31\% &                +59.27\% &              9 &             7 &              +2 \\
% UserKNN CFCBF   &         0.2160 & 0.1680 & 0.2218 &        0.1207 & 0.0650 & 0.1577 &  0.1972 &               +156.16\% &                +52.52\% &              7 &            12 &              -5 \\
% \bottomrule
% \end{tabular}

% }
%     \caption{Comparison of the MovieLens 1M accuracy metrics with single row and Carousel evaluation, both @10. For each evaluation mode, the MAP difference with the base model (TopPop) is shown for each algorithm. Entries are sorted according to the Carousel MAP ranking. \nico{TODO ASSICURARSI CHE I NOMI IN TAB SIANO CONSISTENTI CON I NOMI DATI NELLA SEZ DI DESCRIZIONE}}
%     \label{tab:ml1macc}
% \end{table}

% \begin{table}[]
%     \centering
% \begin{tabular}{l|ccccc|cccc|}
% \toprule
% {} & \multicolumn{5}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} \\
% {} &        Novelty & \begin{tabular}{@{}c@{}}Div. \\ MIL\end{tabular} & \begin{tabular}{@{}c@{}}Cov. \\ Item\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Gini\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Shannon\end{tabular} &       Novelty & \begin{tabular}{@{}c@{}}Cov. \\ Item\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Gini\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Shannon\end{tabular} \\
% \midrule
% TopPop          &         0.0222 &                    0.5541 &        0.0258 &         0.0058 &          4.8398 &        0.0443 &        0.0258 &         0.0058 &          4.8398 \\
% \midrule
% UserKNN CF      &         0.0242 &                    0.9397 &        0.2787 &         0.0585 &          8.1758 &        0.0464 &        0.2750 &         0.0348 &          7.0946 \\
% ItemKNN CF      &         0.0241 &                    0.9325 &        0.2578 &         0.0508 &          7.9752 &        0.0462 &        0.2526 &         0.0311 &          6.9832 \\
% P3alpha         &         0.0239 &                    0.9127 &        0.1651 &         0.0408 &          7.6477 &        0.0461 &        0.1651 &         0.0270 &          6.8534 \\
% RP3beta         &         0.0242 &                    0.9261 &        0.2720 &         0.0519 &          7.9574 &        0.0463 &        0.2720 &         0.0328 &          7.0094 \\
% \midrule
% \EASER          &         0.0238 &                    0.9216 &        0.1859 &         0.0419 &          7.7168 &        0.0460 &        0.1859 &         0.0269 &          6.8480 \\
% SLIM BPR        &         0.0237 &                    0.8929 &        0.2029 &         0.0355 &          7.4008 &        0.0458 &        0.2029 &         0.0241 &          6.6797 \\
% SLIM EN &         0.0244 &                    0.9458 &        0.2913 &         0.0682 &          8.3767 &        0.0466 &        0.2913 &         0.0412 &          7.2517 \\
% \midrule
% MF BPR          &         0.0239 &                    0.9196 &        0.2395 &         0.0474 &          7.8280 &        0.0461 &        0.2395 &         0.0304 &          6.9194 \\
% MF FunkSVD      &         0.0243 &                    0.9473 &        0.2220 &         0.0594 &          8.2414 &        0.0465 &        0.2220 &         0.0360 &          7.1730 \\
% PureSVD         &         0.0243 &                    0.9512 &        0.1965 &         0.0581 &          8.2358 &        0.0465 &        0.1965 &         0.0346 &          7.1676 \\
% NMF             &         0.0248 &                    0.9589 &        0.2261 &         0.0708 &          8.5112 &        0.0469 &        0.2266 &         0.0420 &          7.3865 \\
% IALS            &         0.0246 &                    0.9611 &        0.2640 &         0.0769 &          8.6266 &        0.0468 &        0.2640 &         0.0445 &          7.3981 \\
% \midrule
% ItemKNN CBF     &         0.0289 &                    0.9009 &        0.1808 &         0.0371 &          7.4920 &        0.0510 &        0.1960 &         0.0297 &          7.0807 \\
% UserKNN CBF     &         0.0224 &                    0.6821 &        0.0500 &         0.0083 &          5.3757 &        0.0445 &        0.0502 &         0.0082 &          5.3531 \\
% ItemKNN CFCBF   &         0.0242 &                    0.9381 &        0.2629 &         0.0546 &          8.0872 &        0.0463 &        0.2629 &         0.0338 &          7.0818 \\
% UserKNN CFCBF   &         0.0239 &                    0.9218 &        0.2171 &         0.0430 &          7.7455 &        0.0460 &        0.2174 &         0.0276 &          6.8668 \\
% \bottomrule
% \end{tabular}

%     \caption{MovieLens 1M beyond accuracy metrics according to Individual and Carousel evaluation.}
%     \label{tab:ml1mbeyondacc}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/ml1m_ranking_plot_thres_2.pdf}
%     \caption{Major differences in the ranking of algorithms according to the MAP evaluated in the two different modalities for MovieLens 1M.
%     \nico{da capire quali algoritmi selezionale}}
%     \label{fig:ml1m_ranking}
% \end{figure}

% \begin{figure*}[]
%     \centering
%     \begin{minipage}{.49\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{images/Movielens1M_subplot_beyond_acc.pdf}
%         \caption{Plot of the MAP (Individual and Carousel evaluation) of collaborative algorithms on MovieLens1M with respect to novelty and diversity metrics.}
%         \label{fig:ml1m_plots}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.49\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth]{images/Movielens1M_subplot_beyond_acc_NDCG.pdf}
%         \caption{Plot of the NDCG (Individual and Carousel 2D evaluation) of collaborative algorithms on MovieLens1M with respect to novelty and diversity metrics.}
%         \label{fig:ml1m_ndcg_plots}
%     \end{minipage}
%     \caption{\nico{sembrano troppo piccoli, ingrandire font}}
% \end{figure*}









% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual
% %carousel with 10 items\nico{titolo lungo}
% } & \multicolumn{4}{c|}{Carousel (TopPop)
% %Two carousels with 10 items each
% } &  \multicolumn{2}{c|}{Improvement on TopPop} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.0488 & 0.0527 & 0.0983 &  0.0946 &                  0.00\% &                  0.00\% &             14 &            17 &              -3 \\
% TopPop Drama       &         0.0685 & 0.0499 & 0.0766 &        0.0646 & 0.0575 & 0.1109 &  0.1141 &                -29.63\% &                 +9.04\% &             15 &            14 &              +1 \\
% TopPop new releases &         0.0082 & 0.0043 & 0.0050 &        0.0528 & 0.0541 & 0.1007 &  0.0986 &                -93.88\% &                 +2.67\% &             17 &            16 &              +1 \\
% \midrule
% UserKNN CF          &         0.2343 & 0.2251 & 0.2815 &        0.1338 & 0.0889 & 0.1911 &  0.2492 &               +217.53\% &                +68.59\% &              2 &             5 &              -3 \\
% ItemKNN CF          &         0.1885 & 0.1728 & 0.2122 &        0.1164 & 0.0812 & 0.1662 &  0.2093 &               +143.85\% &                +54.00\% &              9 &            10 &              -1 \\
% \palpha             &         0.1646 & 0.1414 & 0.1915 &        0.0897 & 0.0687 & 0.1451 &  0.1710 &                +99.47\% &                +30.29\% &             13 &            13 &               0 \\
% \pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1104 & 0.0779 & 0.1632 &  0.2035 &               +137.81\% &                +47.83\% &             10 &            11 &              -1 \\
% \midrule
% \EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1281 & 0.0855 & 0.1799 &  0.2293 &               +192.10\% &                +62.10\% &              5 &             8 &              -3 \\
% SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1291 & 0.0872 & 0.1868 &  0.2414 &               +204.64\% &                +65.40\% &              3 &             7 &              -4 \\
% SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        0.1399 & 0.0915 & 0.1931 &  0.2530 &               +230.21\% &                +73.48\% &              1 &             2 &              -1 \\
% \midrule
% MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1088 & 0.0773 & 0.1581 &  0.1932 &               +111.85\% &                +46.66\% &             12 &            12 &               0 \\
% MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1327 & 0.0884 & 0.1859 &  0.2373 &               +146.64\% &                +67.71\% &              8 &             6 &              +2 \\
% PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1329 & 0.0890 & 0.1824 &  0.2357 &               +190.59\% &                +68.74\% &              6 &             4 &              +2 \\
% NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1319 & 0.0895 & 0.1792 &  0.2281 &               +127.51\% &                +69.76\% &             11 &             3 &              +8 \\
% IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1425 & 0.0942 & 0.1895 &  0.2446 &               +203.64\% &                +78.75\% &              4 &             1 &              +3 \\
% \midrule
% ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.0541 & 0.0544 & 0.1022 &  0.1007 &                -92.63\% &                 +3.15\% &             16 &            15 &              +1 \\
% \midrule
% ItemKNN CFCBF       &         0.1950 & 0.1787 & 0.2151 &        0.1198 & 0.0827 & 0.1696 &  0.2148 &               +152.06\% &                +56.77\% &              7 &             9 &              -2 \\
% \bottomrule
% \end{tabular}
% }
%     \caption{Comparison of the MovieLens 10M accuracy metrics with individual and carousel evaluation at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the TopPop carousel is computed with MAP. \nico{senza discussione su ndcg i toppop modificati diventano poco rilevanti}}
%     \label{tab:ml10macc}
% \end{table}


% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel (SLIM)} &  \multicolumn{2}{c|}{Improvement on SLIM} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.1399 & 0.1895 & 0.2967 &  0.2939 &                         -69.72\% &                          +4.81\% &             14 &            13 &              +1 \\
% TopPop Drama       &         0.0685 & 0.0499 & 0.0766 &        0.1372 & 0.1880 & 0.2956 &  0.2921 &                         -78.69\% &                          +3.97\% &             15 &            14 &              +1 \\
% TopPop new releases &         0.0508 & 0.0317 & 0.0392 &        0.1363 & 0.1874 & 0.2936 &  0.2878 &                         -86.47\% &                          +3.67\% &             16 &            15 &              +1 \\
% \midrule
% UserKNN CF          &         0.2343 & 0.2251 & 0.2815 &        0.1528 & 0.1955 & 0.3137 &  0.3225 &                          -3.84\% &                          +8.14\% &              2 &             3 &              -1 \\
% ItemKNN CF          &         0.1885 & 0.1728 & 0.2122 &        0.1455 & 0.1921 & \underline{0.3015} &  \underline{0.3034} &                         -26.15\% &                          +6.27\% &              9 &             9 &               0 \\
% \palpha             &         0.1646 & 0.1414 & 0.1915 &        0.1433 & 0.1912 & 0.3009 &  0.3021 &                         -39.59\% &                          +5.72\% &             13 &            10 &              +3 \\
% \pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1430 & 0.1908 & 0.3014 &  0.3026 &                         -27.98\% &                          +5.50\% &             10 &            11 &              -1 \\
% \midrule
% \EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1430 & 0.1899 & \underline{0.3017} &  \underline{0.3012} &                         -11.54\% &                          +5.06\% &              5 &            12 &              -7 \\
% SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1490 & 0.1937 & 0.3084 &  0.3138 &                          -7.74\% &                          +7.15\% &              3 &             6 &              -3 \\
% SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        0.1230 & 0.1808 & 0.2856 &  0.2734 &                           0.00\% &                           0.00\% &              1 &            17 &             -16 \\
% \midrule
% MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1479 & 0.1937 & 0.3040 &  0.3069 &                         -35.84\% &                          +7.16\% &             12 &             5 &              +7 \\
% MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1560 & 0.1979 & 0.3148 &  0.3248 &                         -25.31\% &                          +9.47\% &              8 &             2 &              +6 \\
% PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1471 & 0.1924 & 0.3039 &  0.3061 &                         -12.00\% &                          +6.43\% &              6 &             7 &              -1 \\
% NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1484 & 0.1938 & 0.3037 &  0.3064 &                         -31.10\% &                          +7.16\% &             11 &             4 &              +7 \\
% IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1592 & 0.1998 & 0.3101 &  0.3174 &                          -8.05\% &                         +10.50\% &              4 &             1 &              +3 \\
% \midrule
% ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.1264 & 0.1826 & 0.2875 &  0.2765 &                         -97.77\% &                          +0.98\% &             17 &            16 &              +1 \\
% \midrule
% ItemKNN CFCBF       &         0.1952 & 0.1790 & 0.2174 &        0.1460 & 0.1923 & 0.3021 &  0.3044 &                         -23.50\% &                          +6.38\% &              7 &             8 &              -1 \\
% \bottomrule
% \end{tabular}
%     }
    
%               \caption{Comparison of the MovieLens10M accuracy metrics with individual and carousel evaluation (with SLIM EN fixed as the first carousel) at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the SLIM EN carousel is computed with MAP.
%               \nico{senza discussione su ndcg i toppop modificati diventano poco rilevanti}}
%     \label{tab:ml10macc_slim}
% \end{table}

% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel (SLIM EN)} &  \multicolumn{2}{c|}{Improvement on SLIM EN} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.1399 & 0.1895 & 0.2967 &  0.2939 &                         -69.72\% &                          +4.81\% &             14 &            13 &              +1 \\
% \midrule
% UserKNN CF          &         0.2343 & 0.2251 & 0.2815 &        0.1528 & 0.1955 & 0.3137 &  0.3225 &                          -3.84\% &                          +8.14\% &              2 &             3 &              -1 \\
% ItemKNN CF          &         0.1885 & 0.1728 & 0.2122 &        0.1455 & 0.1921 & \underline{0.3015} &  \underline{0.3034} &                         -26.15\% &                          +6.27\% &              9 &             9 &               0 \\
% \palpha             &         0.1646 & 0.1414 & 0.1915 &        0.1433 & 0.1912 & 0.3009 &  0.3021 &                         -39.59\% &                          +5.72\% &             13 &            10 &              +3 \\
% \pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1430 & 0.1908 & 0.3014 &  0.3026 &                         -27.98\% &                          +5.50\% &             10 &            11 &              -1 \\
% \midrule
% \EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1430 & 0.1899 & \underline{0.3017} &  \underline{0.3012} &                         -11.54\% &                          +5.06\% &              5 &            12 &              -7 \\
% SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1490 & 0.1937 & 0.3084 &  0.3138 &                          -7.74\% &                          +7.15\% &              3 &             6 &              -3 \\
% SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        0.1230 & 0.1808 & 0.2856 &  0.2734 &                           0.00\% &                           0.00\% &              1 &            15 &             -14 \\
% \midrule
% MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1479 & 0.1937 & 0.3040 &  0.3069 &                         -35.84\% &                          +7.16\% &             12 &             5 &              +7 \\
% MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1560 & 0.1979 & 0.3148 &  0.3248 &                         -25.31\% &                          +9.47\% &              8 &             2 &              +6 \\
% PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1471 & 0.1924 & 0.3039 &  0.3061 &                         -12.00\% &                          +6.43\% &              6 &             7 &              -1 \\
% NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1484 & 0.1938 & 0.3037 &  0.3064 &                         -31.10\% &                          +7.16\% &             11 &             4 &              +7 \\
% IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1592 & 0.1998 & 0.3101 &  0.3174 &                          -8.05\% &                         +10.50\% &              4 &             1 &              +3 \\
% \midrule
% ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.1264 & 0.1826 & 0.2875 &  0.2765 &                         -97.77\% &                          +0.98\% &             15 &            14 &              +1 \\
% \midrule
% ItemKNN CFCBF       &         0.1952 & 0.1790 & 0.2174 &        0.1460 & 0.1923 & 0.3021 &  0.3044 &                         -23.50\% &                          +6.38\% &              7 &             8 &              -1 \\
% \bottomrule
% \end{tabular}
%     }
    
%               \caption{Comparison of the MovieLens10M accuracy metrics with individual and carousel evaluation (with SLIM EN fixed as the first carousel) at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the SLIM EN carousel is computed with MAP.}
%     \label{tab:ml10macc_slim}
% \end{table}

% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on SLIM EN} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        -- & -- & -- &  -- &                           -- &                           -- &              1 &            -- &             -- \\
% \midrule
% \midrule
% TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.1399 & 0.1895 & 0.2967 &  0.2939 &                         -69.7\% &                          +4.8\% &             14 &            13 &              +1 \\
% \midrule
% UserKNN CF          &         0.2343 & 0.2251 & 0.2815 &        0.1528 & 0.1955 & 0.3137 &  0.3225 &                          -3.8\% &                          +8.1\% &              2 &             3 &              -1 \\
% ItemKNN CF          &         0.1885 & 0.1728 & 0.2122 &        0.1455 & 0.1921 & 0.3015 &  0.3034 &                         -26.2\% &                          +6.3\% &              9 &             9 &               0 \\
% \palpha             &         0.1646 & 0.1414 & 0.1915 &        0.1433 & 0.1912 & 0.3009 &  0.3021 &                         -39.6\% &                          +5.7\% &             13 &            10 &              +3 \\
% \pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1430 & 0.1908 & 0.3014 &  0.3026 &                         -28.0\% &                          +5.5\% &             10 &            11 &              -1 \\
% \midrule
% \EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1430 & 0.1899 & 0.3017 &  0.3012 &                         -11.5\% &                          +5.1\% &              5 &            12 &              -7 \\
% SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1490 & 0.1937 & 0.3084 &  0.3138 &                          -7.7\% &                          +7.2\% &              3 &             6 &              -3 \\
% \midrule
% MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1479 & 0.1937 & 0.3040 &  0.3069 &                         -35.8\% &                          +7.2\% &             12 &             5 &              +7 \\
% MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1560 & 0.1979 & 0.3148 &  0.3248 &                         -25.3\% &                          +9.5\% &              8 &             2 &              +6 \\
% PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1471 & 0.1924 & 0.3039 &  0.3061 &                         -12.0\% &                          +6.4\% &              6 &             7 &              -1 \\
% NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1484 & 0.1938 & 0.3037 &  0.3064 &                         -31.1\% &                          +7.2\% &             11 &             4 &              +7 \\
% IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1592 & 0.1998 & 0.3101 &  0.3174 &                          -8.1\% &                         +10.5\% &              4 &             1 &              +3 \\
% \midrule
% ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.1264 & 0.1826 & 0.2875 &  0.2765 &                         -97.8\% &                          +1.0\% &             15 &            14 &              +1 \\
% \midrule
% ItemKNN CFCBF       &         0.1952 & 0.1790 & 0.2174 &        0.1460 & 0.1923 & 0.3021 &  0.3044 &                         -23.5\% &                          +6.4\% &              7 &             8 &              -1 \\
% \bottomrule
% \end{tabular}
%     }
    
%               \caption{Comparison of the MovieLens10M accuracy metrics with individual and carousel evaluation (with SLIM EN fixed as the first carousel) at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the SLIM EN carousel is computed with MAP.}
%     \label{tab:ml10macc_slim}
% \end{table}

% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on SLIM EN} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        -- & -- & -- &  -- &                           -- &                           -- &              -- &            -- &             -- \\
% \midrule
% \midrule
% TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.1399 & 0.1895 & 0.2967 &  0.2939 &                         -69.7\% &                          +4.8\% &             13 &            13 &              0 \\
% \midrule
% UserKNN CF          &         0.2343 & 0.2251 & 0.2815 &        0.1528 & 0.1955 & 0.3137 &  0.3225 &                          -3.8\% &                          +8.1\% &              1 &             3 &              -2 \\
% ItemKNN CF          &         0.1885 & 0.1728 & 0.2122 &        0.1455 & 0.1921 & 0.3015 &  0.3034 &                         -26.2\% &                          +6.3\% &              8 &             9 &               -1 \\
% \palpha             &         0.1646 & 0.1414 & 0.1915 &        0.1433 & 0.1912 & 0.3009 &  0.3021 &                         -39.6\% &                          +5.7\% &             12 &            10 &              +2 \\
% \pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1430 & 0.1908 & 0.3014 &  0.3026 &                         -28.0\% &                          +5.5\% &             9 &            11 &              -2 \\
% \midrule
% \EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1430 & 0.1899 & 0.3017 &  0.3012 &                         -11.5\% &                          +5.1\% &              4 &            12 &              -8 \\
% SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1490 & 0.1937 & 0.3084 &  0.3138 &                          -7.7\% &                          +7.2\% &              2 &             6 &              -4 \\
% \midrule
% MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1479 & 0.1937 & 0.3040 &  0.3069 &                         -35.8\% &                          +7.2\% &             11 &             5 &              +6 \\
% MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1560 & 0.1979 & 0.3148 &  0.3248 &                         -25.3\% &                          +9.5\% &              7 &             2 &              +5 \\
% PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1471 & 0.1924 & 0.3039 &  0.3061 &                         -12.0\% &                          +6.4\% &              5 &             7 &              -2 \\
% NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1484 & 0.1938 & 0.3037 &  0.3064 &                         -31.1\% &                          +7.2\% &             10 &             4 &              +6 \\
% IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1592 & 0.1998 & 0.3101 &  0.3174 &                          -8.1\% &                         +10.5\% &              3 &             1 &              +2 \\
% \midrule
% ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.1264 & 0.1826 & 0.2875 &  0.2765 &                         -97.8\% &                          +1.0\% &             14 &            14 &              0 \\
% \midrule
% ItemKNN CFCBF       &         0.1952 & 0.1790 & 0.2174 &        0.1460 & 0.1923 & 0.3021 &  0.3044 &                         -23.5\% &                          +6.4\% &              6 &             8 &              -2 \\
% \bottomrule
% \end{tabular}
%     }
    
%               \caption{Comparison of the MovieLens10M accuracy metrics with individual and carousel evaluation (with SLIM EN fixed as the first carousel) at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the SLIM EN carousel is computed with MAP.}
%     \label{tab:ml10macc_slim}
% \end{table}

\begin{table*}[]
    \centering
    \resizebox{0.94\textwidth}{!}{%
\begin{tabular}{l|ccc|cccc|cc|cc|c|}
\toprule
    {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel (SLIM EN)} &  \multicolumn{2}{c|}{Improvement on SLIM EN} &       \multicolumn{3}{c|}{MAP rank}      \\
{} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
\midrule
SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        -- & -- & -- &  -- &                           -- &                           -- &              -- &            -- &             -- \\
\midrule
\midrule
TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.1399 & 0.1895 & 0.2967 &  0.2939 &                         -69.7\% &                          +4.8\% &             13 &            13 &              0 \\
\midrule
UserKNN CF          &         0.2343 & 0.2251 & 0.2815 &        0.1528 & 0.1955 & 0.3137 &  0.3225 &                          -3.8\% &                          +8.1\% &              1 &             3 &              -2 \\
ItemKNN CF          &         0.1885 & 0.1728 & 0.2122 &        0.1455 & 0.1921 & 0.3015 &  0.3034 &                         -26.2\% &                          +6.3\% &              8 &             9 &               -1 \\
\palpha             &         0.1646 & 0.1414 & 0.1915 &        0.1433 & 0.1912 & 0.3009 &  0.3021 &                         -39.6\% &                          +5.7\% &             12 &            10 &              +2 \\
\pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1430 & 0.1908 & 0.3014 &  0.3026 &                         -28.0\% &                          +5.5\% &             9 &            11 &              -2 \\
\midrule
\EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1430 & 0.1899 & 0.3017 &  0.3012 &                         -11.5\% &                          +5.1\% &              4 &            12 &              -8 \\
SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1490 & 0.1937 & 0.3084 &  0.3138 &                          -7.7\% &                          +7.2\% &              2 &             6 &              -4 \\
\midrule
MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1479 & 0.1937 & 0.3040 &  0.3069 &                         -35.8\% &                          +7.2\% &             11 &             5 &              +6 \\
MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1560 & 0.1979 & 0.3148 &  0.3248 &                         -25.3\% &                          +9.5\% &              7 &             2 &              +5 \\
PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1471 & 0.1924 & 0.3039 &  0.3061 &                         -12.0\% &                          +6.4\% &              5 &             7 &              -2 \\
NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1484 & 0.1938 & 0.3037 &  0.3064 &                         -31.1\% &                          +7.2\% &             10 &             4 &              +6 \\
IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1592 & 0.1998 & 0.3101 &  0.3174 &                          -8.1\% &                         +10.5\% &              3 &             1 &              +2 \\
\midrule
ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.1264 & 0.1826 & 0.2875 &  0.2765 &                         -97.8\% &                          +1.0\% &             14 &            14 &              0 \\
\midrule
ItemKNN CFCBF       &         0.1952 & 0.1790 & 0.2174 &        0.1460 & 0.1923 & 0.3021 &  0.3044 &                         -23.5\% &                          +6.4\% &              6 &             8 &              -2 \\
\bottomrule
\end{tabular}
    }

    \resizebox{0.4\textwidth}{!}{%
    \centering
    \includegraphics[width=\columnwidth]{images/carouselEvalDiagram-4.pdf}
    }
    
    \caption{Comparison of the MovieLens10M accuracy metrics with individual and carousel evaluation (with SLIM EN fixed as the first carousel) at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the SLIM EN carousel is computed with MAP.}
    \label{tab:ml10macc_slim}
\end{table*}

\subsection{Discussion on the results}

% \nico{r2 dice: replicating the baseline model to all carousels doesn’t seem right.} 
% \nico{RISOLTO: tolta da qui, detta nella sezione di risultati e motivata con il fatto che vogliamo misurare l'improvement portato da altri modelli oltre al carosello fissato}
% \nico{Elenco di cose da dire:
%     -- Indagare se c'è una qualche proprietà speciale propria dei metodi matrix factorization, dato che SEMBRA che salgano nel ranking Carousel.
%     -- Forse dovremmo dire qualcosa anche sui risultati NDCG2D, altrimenti la sua definizione potrebbe sembrare inutile.
% }
% \nico{r2 pensa che il TopPop sia una baseline} 
% \nico{RISOLTO: non dovrebbe chiamarsi più baseline da nessuna parte spero}
% \nico{a r3 non è piaciuto il fatto che abbiamo messo nel carosello fisso solo modelli non-personalized, perché: This implies the main findings cannot be generalised to other, more realistic scenarios where the multiple carousels are generated by several "personalised" algorithms.} 
% \nico{RISOLTO: additional material con SLIM}
% \nico{r3 dice: Therefore, I believe papers like this proposing improvements in offline evaluation protocols should include some sort of online evaluation} \nico{RISOLTO: Future work}

For each algorithm, we report both its individual recommendation quality and the evaluation under a carousel setting when the first carousel is fixed and each algorithm is used to fill the second carousel (see Table \ref{tab:ml10macc_slim}). All recommendation lists have a length, \idest cutoff, of 10, however note that in the individual evaluation there will be a single recommendation list while in the carousel evaluation there will be more than one, in this case two. We evaluated two cases, in the first one the fixed carousel is a non-personalized TopPopular model, while in the second it is SLIM EN, the personalized model with the highest individual MAP. %as the fixed carousel on top, and the other with a personalized one. Among the personalized algorithms, we chose the one with the highest individual MAP, which is SLIM EN for both datasets. 
For the NDCG2D, we chose as an example $\alpha=\beta=1$ in which the user explores both horizontally and vertically with equivalent penalty. 
% As an example, in the following, we show and discuss only the results for MovieLens10M with a TopPop carousel fixed (Table \ref{tab:ml10macc}).
The results obtained with the TopPop and SLIM EN fixed carousels and for both datasets are broadly similar. For space reasons we will only discuss the results for MovieLens10M with a SLIM EN fixed carousel (see Table \ref{tab:ml10macc_slim}). We provide the full results in the online material.
% Many observations made for this scenario are valid and consistent with the other scenarios' results, which we provide in the additional material. \nico{fornire referenza al materiale}
% Since the objective of the carousel evaluation is to understand how other models improve the performance of the fixed model alone, we filled the second carousel with non-relevant recommendations when evaluating the fixed carousel. \nico{forse un po' contorta ma non so come dirlo.}

%The results for the MovieLens 10M dataset are reported in Table \ref{tab:ml10macc}. % and \ref{tab:ml10mbeyondacc} (beyond-accuracy metrics). %describe the performance of the various algorithms on the MovieLens 10M dataset, according to accuracy and beyond accuracy metrics, respectively. 
 %the evaluation on both the standard Individual evaluation and the novel carousel evaluation. 
% By looking at Table \ref{tab:ml10macc} we can make several considerations. 
%Under the traditional evaluation in which an algorithm is evaluated independently (\idest individual) we can see that almost all algorithms have a recommendation quality between two and three times better than TopPop. The best performing algorithms are SLIM, UserKNN and IALS.
%W
% Looking at the results for MovieLens 10M (Table \ref{tab:ml10macc}),
% Looking at the results,
% we can see that almost all algorithms have a recommendation quality between two and three times better than TopPop under the traditional individual evaluation. The best performing algorithms are SLIM, UserKNN and IALS.
% %Only the ItemKNN CBF performs worse than TopPop.
% For the carousel evaluation, 
% % we can see that no algorithm has a lower recommendation quality than TopPop, which is expected since TopPop is the predefined first carousel while each algorithm is the second one and therefore the final recommendation quality can only be greater or equal. Due to this, even the poorly performing ItemKNN CBF produces an improvement over the TopPop baseline of 3.15\%. If we look at the improvement of MAP of the algorithms over the TopPop baseline we can see that in the carousel evaluation the difference is still wide but smaller. This is because the personalized models only fill half of the entire set of recommendations provided to the user and the evaluation only measures the \emph{new} correct recommendations the personalized model allows. 
% %we can see that 
% the difference of MAP of the algorithms over the TopPop carousel is still wide but smaller. This is because the personalized models only fill half of the entire set of recommendations provided to the user and the evaluation only measures the \emph{new} correct recommendations the personalized model allows. 


% % \begin{table}[]
% % \footnotesize
% %     \centering
% % \begin{tabular}{l|ccccccc|}
% % \toprule
% % {} & \multicolumn{7}{c|}{Individual} \\
% % {} &        Novelty & \begin{tabular}{@{}c@{}}Div. \\ MIL\end{tabular} & \begin{tabular}{@{}c@{}}Cov. \\ Item\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Gini\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Shannon\end{tabular} & \begin{tabular}{@{}c@{}}Cov. \\ Item \\ Correct\end{tabular} & \begin{tabular}{@{}c@{}}Avg. \\ Popularity\end{tabular} \\
% % \midrule
% % TopPop                 &         0.0079 &                    0.5369 &        0.0124 &         0.0020 &          4.7635 &                0.0121 &             0.8112 \\
% % TopPop Drama          &         0.0082 &                    0.4668 &        0.0110 &         0.0017 &          4.4866 &                0.0105 &             0.6856 \\
% % TopPop new releases    &         0.0108 &                    0.0840 &        0.0078 &         0.0011 &          3.6049 &                0.0070 &             0.0951 \\
% % \midrule
% % UserKNN CF             &         0.0089 &                    0.9491 &        0.2464 &         0.0262 &          8.4579 &                0.1348 &             0.4535 \\
% % ItemKNN CF             &         0.0086 &                    0.9029 &        0.1490 &         0.0118 &          7.3419 &                0.0913 &             0.5248 \\
% % P3alpha                &         0.0083 &                    0.8012 &        0.0606 &         0.0059 &          6.3318 &                0.0490 &             0.6751 \\
% % RP3beta                &         0.0086 &                    0.8941 &        0.1680 &         0.0117 &          7.2875 &                0.0977 &             0.5584 \\
% % \midrule
% % EASE R                 &         0.0086 &                    0.9221 &        0.1020 &         0.0144 &          7.6602 &                0.0804 &             0.5326 \\
% % SLIM BPR               &         0.0089 &                    0.9416 &        0.2055 &         0.0232 &          8.2771 &                0.1368 &             0.4750 \\
% % SLIM EN        &         0.0090 &                    0.9491 &        0.2477 &         0.0294 &          8.5653 &                0.1799 &             0.4567 \\
% % \midrule
% % MF BPR                 &         0.0088 &                    0.9348 &        0.2040 &         0.0217 &          8.1467 &                0.1304 &             0.4957 \\
% % MF FunkSVD             &         0.0094 &                    0.9762 &        0.1866 &         0.0460 &          9.3491 &                0.1597 &             0.3533 \\
% % PureSVD                &         0.0088 &                    0.9428 &        0.0885 &         0.0174 &          7.9644 &                0.0846 &             0.4865 \\
% % NMF                    &         0.0091 &                    0.9591 &        0.1060 &         0.0236 &          8.4094 &                0.0983 &             0.3826 \\
% % IALS                   &         0.0090 &                    0.9629 &        0.1676 &         0.0300 &          8.7295 &                0.1584 &             0.4255 \\
% % \midrule
% % ItemKNN CBF &         0.0134 &                    0.9680 &        0.4663 &         0.0511 &          9.3030 &                0.0485 &             0.0692 \\
% % \midrule
% % ItemKNN CFCBF  &         0.0087 &                    0.9236 &        0.2078 &         0.0156 &          7.7111 &                0.1129 &             0.5047 \\
% % \bottomrule
% % \end{tabular}

% %     \caption{MovieLens 10M beyond accuracy metrics according to the individual evaluation. Cov. Item Correct reports the Item Coverage only considering correct recommendations.}
% %     \label{tab:ml10mbeyondacc}
% % \end{table}

% As a general trend we can see that the relative performance of the models differ, resulting in changes to the ranking of the algorithms in the two evaluation modes. Some models 
% %such as \palpha and MF BPR
% %are ranked in the same position. Others
% , in this case all other matrix factorization algorithms, gain 2 or 3 positions with the exception of NMF that jumps up by 8 positions becoming the 3\textsuperscript{rd} best model. On the other hand, KNNs, graph-based and item-based machine learning models tend to lose some positions. As a result,
% %while in the individual evaluation the best algorithms are SLIM EN, UserKNN and SLIM BPR,
% in the carousel evaluation the best algorithms are IALS, SLIM EN and NMF.
% %Since the recommendation lists generated by all algorithms are identical for both evaluation procedures, t
% The difference in those rankings lies in how those recommendations intersect. Algorithms which will tend to recommend popular items will be penalized in this carousel evaluation because popular items will already be present in the TopPop carousel, whereas algorithms providing accurate recommendation but involving less popular items will be advantaged. 



%We can compare the two rankings by computing the Kendall $\tau$ coefficient, which represents the quota of algorithms that are in the same relative position. For the MovieLens 10M dataset with the TopPop carousel the Kendall $\tau$ coefficient is 0.67, indicating that the two rankings are quite different.
%The changes can be more easily seen in Figure \ref{fig:ml10m_ranking}.
% Table \ref{tab:ml10mbeyondacc} reports common beyond-accuracy metrics for the individual evaluation.
% We computed a set of common beyond-accuracy metrics for the individual evaluation, described in Section \ref{sec:evaluation_metrics} which are not reported here for space reasons. There emerges no clear pattern that connects the diversity of the individual model to how well it will perform in the carousel evaluation setting, further pointing to the importance of accounting for the interactions between the recommendation lists. Further analysis could highlight patterns that could be exploited as heuristics for the selection of optimal carousels. We leave this as an open research question.





% As it can be seen from the Individual MAP rank column of Table \ref{tab:ml10macc}, the best MAP evaluated independently is provided by SLIM EN. This is not consistent, though, with our carousel evaluation protocol, where the same algorithm is 2\textsuperscript{nd}. In fact, considering also the interactions among carousels, it can be observed how IALS is the best choice for the streaming service provider. 
% In general, looking at the difference between the rankings in the two evaluation protocols shown in the $\Delta$ MAP rank column, we can notice how many algorithms have different positions in the global ranking. Particularly relevant is the example of NMF, which from 11\textsuperscript{th} place reaches the 3\textsuperscript{rd} one. A proof of the difference between the two rankings is the fact that Kendall's $\tau$ coefficient of those is 0.67. This suggests that the two rankings are somehow correlated (as expected), but the fact that $\tau$ < 1 means that the Individual ranking is not sufficient to make any conclusion about the carousel MAP ranking. \nico{non so se le conclusioni da trarre da Kendall sono giuste} Therefore, this is another proof of the necessity of a novel evaluation protocol.  A visualization of the major differences between the two rankings is provided in Fig. \ref{fig:ml10m_ranking}.

% For instance, looking at the $\Delta_{TopPop}$ MAP column, we can notice how a standard Individual evaluation could be non-realistic in a carousel scenario. Indeed, if we take the ItemKNN CBF, we can see how this algorithm seemed to have much lower performance (MAP) with respect to the simple TopPop, both evaluated independently. Instead, if a carousel evaluation approach is adopted, it overperforms the TopPop by 3.15\%. This happens because of the different natures of the TopPop, which takes in input solely items popularities, and the ItemKNN CBF, which exploits content information in order to make recommendations. In a scenario where the TopPop carousel is fixed as the top carousel due to business constraints, such a different point of view translates to an improvement of the user experience. This improvement could not be foreseen with the standard evaluation mode.

% As a general trend, we notice how the $\Delta_{TopPop}$ MAP always presents differences in the two evaluation modalities, but this was expected since we fixed a TopPop carousel above every algorithm's recommendation list in the carousel evaluation. The interesting aspect, though, is that this difference is not consistent with the performance of the algorithms evaluated independently. Indeed, let us take as examples ItemKNN CF and MF FunkSVD algorithms. Evaluated independently, they provide an improvement (with respect to the TopPop independent evaluation) of +151.19\% and +146.64\%, respectively. Instead, with the carousel evaluation, the improvement becomes of +54.00\% and +67.71\%, respectively.


% Apart from the single example, we can notice a general trend from these data: the $\Delta_{TopPop}$ MAP presents always differences in the two evaluation modalities. \nico{TODO il fatto che siano diverse e' atteso, dato che nel carousel evaluation c'e' un carosello TopPop fisso prima dell'algoritmo, che quindi ci fa pensare ad una diminuzione delle performance. L'aspetto da notare e' come il cambiamento di performance non sia consistente con le performance degli algoritmi valutate indipendentemente. Basta fare due esempi di scambio ranking.}

% Hence, we believe that our evaluation procedure is necessary for real scenarios with carousels that we described before since it sheds light on hidden interactions among carousels that could not be visible with a standard evaluation approach. \nico{questi ultimi due paragrafi forse sono ridondanti con il prossimo paragrafo che parla del ranking.}

% As further evidence of this, let us consider the situation where the provider of a streaming service homepage formed of carousels, with a fixed TopPop carousel on the top of the page, has to choose which algorithm's carousel present to the users. To do so, she could naively select the best performing algorithm according to some metric (let us assume it is MAP) with the standard Individual evaluation. As it can be seen from the Individual MAP rank column of Table \ref{tab:ml10macc}, the best MAP evaluated independently is provided by SLIM EN. This is not consistent, though, with our carousel evaluation protocol, where the same algorithm is 2\textsuperscript{nd}. In fact, considering also the interactions among carousels, it can be observed how IALS is the best choice for the streaming service provider. 
% In general, looking at the difference between the rankings in the two evaluation protocols shown in the $\Delta$ MAP rank column, we can notice how many algorithms have different positions in the global ranking. Particularly relevant is the example of NMF, which from 11\textsuperscript{th} place reaches the 3\textsuperscript{rd} one. A proof of the difference between the two rankings is the fact that Kendall's $\tau$ coefficient of those is 0.67. This suggests that the two rankings are somehow correlated (as expected), but the fact that $\tau$ < 1 means that the Individual ranking is not sufficient to make any conclusion about the carousel MAP ranking. \nico{non so se le conclusioni da trarre da Kendall sono giuste} Therefore, this is another proof of the necessity of a novel evaluation protocol.  A visualization of the major differences between the two rankings is provided in Fig. \ref{fig:ml10m_ranking}.

% These results seem to suggest some common patterns regarding which algorithms will perform better or less so in a carousel evaluation with TopPopular carousel.
% In Figure \ref{fig:ml10m_plots} and \ref{fig:ml10m_ndcg_plots}, we plot both MAP and NDCG metrics in the Individual evaluation compared to MIL diversity and Novelty metrics.\footnote{Due to their low recommendation quality with both evaluation protocols, we excluded from the plot the ItemKNN CBF and TopPopular algorithms.}
% For each of those plots, the trend line is shown as a red dashed line. \mf{provare a mettere modello lineare e riportare correlazione con spearman o kendall, includere coverage item correct} Such a trend line is computed as the least-squares fit of the various points on the plot for a second order polynomial. From Figure \ref{fig:ml10m_plots} we can see that in the Individual evaluation, many algorithms exhibit a high MIL diversity (above 0.90) but there seems to be no relation to the corresponding MAP and NDCG value. However, under the carousel evaluation the best performing models are more concentrated towards higher diversity values. \mf{rivedere} This observation is consistent with the finding that popularity biased algorithms may hamper the effectiveness of a recommender model in a real scenario, and hence the user experience \cite{DBLP:conf/recsys/AbdollahpouriMB19}. Furthermore, this behavior agrees with previous observations on how a set of diverse and novel recommendations are beneficial \cite{chen2018fast,DBLP:conf/recsys/ZhangH08}. 
% \mf{note su diversity, da sola non basta}




% \begin{table}[]
%     \centering
%     \footnotesize
% \begin{tabular}{l|c|cc|cc|cc|}
% \toprule
% {} & {} & \multicolumn{2}{c|}{TopPop Drama}  & \multicolumn{2}{c|}{TopPop new releases} & \multicolumn{2}{c|}{ItemKNN CBF} \\
% {} &       Individual &      Carousel & $ \Delta $ rank &      Carousel & $ \Delta $ rank &      Carousel & $ \Delta $ rank \\
% \midrule
% TopPop               &             14 &            14 &               0 &            14 &               0 &            14 &               0 \\
% TopPop Drama        &             15 &            17 &              -2 &            15 &               0 &            15 &               0 \\
% TopPop new releases  &             17 &            16 &              +1 &            17 &               0 &            16 &              +1 \\
% \midrule
% UserKNN CF    &              2 &             3 &              -1 &             2 &               0 &             2 &               0 \\
% ItemKNN CF    &              9 &            10 &              -1 &             9 &               0 &             9 &               0 \\
% \palpha              &             13 &            13 &               0 &            13 &               0 &            13 &               0 \\
% \pbeta              &             10 &            11 &              -1 &            10 &               0 &            10 &               0 \\
% \midrule
% \EASER               &              5 &             6 &              -1 &             5 &               0 &             5 &               0 \\
% SLIM BPR             &              3 &             4 &              -1 &             4 &              -1 &             4 &              -1 \\
% SLIM EN      &              1 &             2 &              -1 &             1 &               0 &             1 &               0 \\
% \midrule
% MF BPR               &             12 &            12 &               0 &            12 &               0 &            12 &               0 \\
% MF FunkSVD           &              8 &             7 &              +1 &             8 &               0 &             8 &               0 \\
% PureSVD              &              6 &             5 &              +1 &             6 &               0 &             6 &               0 \\
% NMF                  &             11 &             8 &              +3 &            11 &               0 &            11 &               0 \\
% IALS                 &              4 &             1 &              +3 &             3 &              +1 &             3 &              +1 \\
% \midrule
% ItemKNN CBF   &             16 &            15 &              +1 &            16 &               0 &            17 &              -1 \\
% \midrule
% ItemKNN CFCBF &              7 &             9 &              -2 &             7 &               0 &             7 &               0 \\
% \bottomrule
% \end{tabular}

%     \caption{Comparison of the MAP ranking under different carousels in MovieLens10M. The rows indicate which algorithm is used as second carousel, while the first one is, according to the column: TopPop Drama, TopPop new releases or the ItemKNN CBF.
%     }
%     \label{tab:carousels_rank}
% \end{table}




% \nico{forse tagliare} The impact of different variations of the baseline carousel can be seen in Table \ref{tab:carousels_rank}. The first two baseline carousels are variations of the traditional TopPop algorithm, \emph{TopPop Drama} only considers the most popular items of the Drama genre, the one associated to the most items, \emph{TopPop new releases} only considers the most popular items among the movies of the last 2 years. From the previous Table \ref{tab:ml10macc} we can see that those baselines have lower recommendation quality compared to TopPop, with TopPop new releases performing very poorly. This however does not translate into easily predictable changes in the algorithm ranking. Notably, despite TopPop new releases having only a tenth of the recommendation quality of the TopPop Drama, their recommendation quality difference in the carousel evaluation is in the range of 10\%, see Table \ref{tab:ml10macc}.
% This indicates that recommendation quality alone is not sufficient to assess how will a baseline carousel impact the ranking and the interactions between the recommendation lists themselves have to be taken into account. 
% In Table \ref{tab:carousels_rank} we can see the variations in the algorithm ranking if we change the baseline carousel replacing TopPop with TopPop Drama, TopPop new releases and ItemKNN CBF. As the recommendation quality of the first carousel drops, the ranking of the carousel evaluation becomes more similar to that of the individual evaluation. 

%The Kendall $\tau$ coefficient is 0.85 for the TopPop Drama carousel, 0.98 for the TopPop new releases carousel and 0.97 for the ItemKNN CBF carousel.
% Lastly, we also report the results considering as baseline carousel the ItemKNN CBF model. In this case, the ranking of the algorithms is almost identical to the independent evaluation. This could be expected due to the very low recommendation quality of the ItemKNN CBF compared to the other collaborative algorithms. 
% Interestingly, in the experiments we report for MovieLens the similarity-based models that change their ranking consistently lose positions, while the matrix factorization models gain positions. This suggests that the recommendations provided by the matrix factorization algorithms are less similar to the TopPopular ones.

 



% Given these results, we tried to analyze them in order to understand which could be the effect of the interaction among carousels. 
% In Fig. \ref{fig:ml10m_plots} and \ref{fig:ml10m_ndcg_plots}, we show some scatter plots of how MAP and NDCG metrics vary with respect to a beyond accuracy metrics. In particular, we selected the MIL diversity and the Novelty metrics. Due to their poor performance with both evaluation modes, we decided to exclude from the plot the purely content-based, the Random and the TopPop algorithms. \nico{non so se va bene come spiegazione} MAP and NDCG are evaluated following both the standard independent evaluation and the carousel evaluation protocol. For the NDCG, the carousel evaluation is done using our two-dimensional variant. 
% For each of those plots, the trend line is shown as a red dashed line. Such a trend line is computed as the least-squares polynomial fit of the various points on the plot. The implementation used is NumPy \texttt{polyfit} function\footnote{\url{https://numpy.org/doc/stable/reference/generated/numpy.polyfit.html}}. The degree of the polynomial is two.
% Looking at those plots, it becomes clear how the beyond accuracy metrics are positively correlated with the carousel accuracy, while there was little to no correlation with the accuracy evaluated independently. 
% This result is noteworthy because it shows how, in a real scenario with carousels, the choice of which recommendation lists display should take into account how those lists complement each other. Therefore, lists that provide diversity or novelty may be beneficial when a TopPop carousel is fixed above them, given the alternative perspective they bring. Also, this provides another evidence of how popularity biased algorithms may harm the user experience in real scenarios \cite{DBLP:conf/recsys/AbdollahpouriMB19}. Furthermore, this result is consistent with previous observations on how a set of diverse and novel recommendations may improve user satisfaction \cite{chen2018fast, DBLP:conf/recsys/ZhangH08}. 

% \nico{Preso da uno delle contribution nell'intro: An indication that the carousel evaluation protocol produces results consistent with previous observations in A/B testing \mf{diversity is better, cit. Verificare}}


% The results for the Netflix dataset are reported in Table \ref{tab:netflix_acc} \nico{dire dove abbiamo messo la tabella per motivi di spazio}. Compared to MovieLens 10M we can observe that the TopPopular algorithm has a similar recommendation quality gap with the personalized algorithms. This, however, has a smaller impact on the relative ranking of the algorithms. Interestingly, as observed for the MovieLens 10M dataset, the similarity based models (both heuristic and machine learning ones) that change their ranking, tend to lose positions.
% %, with the exception of \pbeta.
% Similarly, the matrix factorization algorithms tend to gain positions, in particular IALS. 
% %In this case the position of NMF, that made substantial gains on MovieLens, remains unchanged. Again, both \palpha and MF BPR do not change their ranking.

% Lastly, the results for the Spotify dataset are reported in Table \ref{tab:spotify_acc}. Compared to the other datasets the TopPopular algorithm has very poor recommendation quality. As could be expected, the poor quality of the baseline carousel results in an unaltered ranking. This again confirms that the interactions between recommendation lists have an impact in the resulting recommendation quality and that, while a poorly performing carousel will not impact the relative performance of the models, a well performing one will. As the number of carousels increases, finding another model which is sufficiently different from those already present in the carousels will become an increasingly difficult task.


% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on TopPop} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop              &         0.0975 & 0.0709 & 0.0983 &        0.0488 & 0.0527 & 0.0983 &  0.0946 &                  0.00\% &                  0.00\% &             14 &            17 &              -3 \\
% TopPop Drama      &         0.0685 & 0.0499 & 0.0766 &        0.0646 & 0.0575 & 0.1109 &  0.1141 &                -29.63\% &                 +9.04\% &             15 &            15 &               0 \\
% TopPop new releases \nico{last 10 years, decidere quale tenere} &         0.0508 & 0.0317 & 0.0392 &        0.0722 & 0.0608 & 0.1155 &  0.1233 &                -55.33\% &                +15.25\% &             16 &            14 &              +2 \\
% \midrule
% UserKNN CF          &         0.2375 & 0.2303 & 0.2804 &        0.1338 & 0.0889 & 0.1911 &  0.2492 &               +224.95\% &                +68.59\% &              2 &             5 &              -3 \\
% ItemKNN CF          &         0.1954 & 0.1780 & 0.2121 &        0.1164 & 0.0812 & 0.1662 &  0.2093 &               +151.19\% &                +54.00\% &              8 &            10 &              -2 \\
% \palpha             &         0.1646 & 0.1414 & 0.1915 &        0.0897 & 0.0687 & 0.1451 &  0.1710 &                +99.47\% &                +30.29\% &             13 &            13 &               0 \\
% \pbeta             &         0.1886 & 0.1686 & 0.2160 &        0.1104 & 0.0779 & 0.1632 &  0.2035 &               +137.81\% &                +47.83\% &             10 &            11 &              -1 \\
% \midrule
% \EASER              &         0.2260 & 0.2070 & 0.2566 &        0.1281 & 0.0855 & 0.1799 &  0.2293 &               +192.10\% &                +62.10\% &              5 &             8 &              -3 \\
% SLIM BPR            &         0.2274 & 0.2159 & 0.2699 &        0.1291 & 0.0872 & 0.1868 &  0.2414 &               +204.64\% &                +65.40\% &              3 &             7 &              -4 \\
% SLIM EN     &         0.2460 & 0.2340 & 0.2856 &        0.1399 & 0.0915 & 0.1931 &  0.2530 &               +230.21\% &                +73.48\% &              1 &             2 &              -1 \\
% MF BPR              &         0.1759 & 0.1502 & 0.1882 &        0.1088 & 0.0773 & 0.1581 &  0.1932 &               +111.85\% &                +46.66\% &             12 &            12 &               0 \\
% MF FunkSVD          &         0.2039 & 0.1748 & 0.2307 &        0.1327 & 0.0884 & 0.1859 &  0.2373 &               +146.64\% &                +67.71\% &              9 &             6 &              +3 \\
% PureSVD             &         0.2217 & 0.2060 & 0.2527 &        0.1329 & 0.0890 & 0.1824 &  0.2357 &               +190.59\% &                +68.74\% &              6 &             4 &              +2 \\
% NMF                 &         0.1872 & 0.1613 & 0.1974 &        0.1319 & 0.0895 & 0.1792 &  0.2281 &               +127.51\% &                +69.76\% &             11 &             3 &              +8 \\
% IALS                &         0.2329 & 0.2152 & 0.2539 &        0.1425 & 0.0942 & 0.1895 &  0.2446 &               +203.64\% &                +78.75\% &              4 &             1 &              +3 \\
% \midrule
% ItemKNN CBF         &         0.0113 & 0.0052 & 0.0079 &        0.0541 & 0.0544 & 0.1022 &  0.1007 &                -92.63\% &                 +3.15\% &             17 &            16 &              +1 \\
% \midrule
% ItemKNN CFCBF       &         0.1950 & 0.1787 & 0.2151 &        0.1198 & 0.0827 & 0.1696 &  0.2148 &               +152.06\% &                +56.77\% &              7 &             9 &              -2 \\
% \bottomrule
% \end{tabular}

% }
%     \caption{Comparison of the MovieLens 10M accuracy metrics with single row and carousel evaluation, both @10. For each evaluation mode, the MAP difference with the base model (TopPop) is shown for each algorithm.}
%     \label{tab:ml10macc}
% \end{table}

% \begin{table*}[]
%     \centering
%     \begin{minipage}{.32\textwidth}
%             \centering
%             \resizebox{\columnwidth}{!}{%
%             \begin{tabular}{l|c|c|}
%                 \toprule
%                 {} & \multicolumn{2}{c|}{MAP rank} \\
%                 {} &      \begin{tabular}{@{}c@{}}Carousel \\ (TopPop genre) \end{tabular} & $ \Delta $ rank \\
%                 \midrule
%                 TopPop              &            14 &               0 \\
%                 TopPop genre       &            17 &              -2 \\
%                 TopPop new releases &            15 &              +1 \\
%                 \midrule
%                 UserKNN CF          &             3 &              -1 \\
%                 ItemKNN CF          &            10 &              -2 \\
%                 \palpha             &            13 &               0 \\
%                 \pbeta             &            11 &              -1 \\
%                 \midrule
%                 \EASER              &             6 &              -1 \\
%                 SLIM BPR            &             4 &              -1 \\
%                 SLIM EN     &             2 &              -1 \\
%                 MF BPR              &            12 &               0 \\
%                 MF FunkSVD          &             7 &              +2 \\
%                 PureSVD             &             5 &              +1 \\
%                 NMF                 &             8 &              +3 \\
%                 IALS                &             1 &              +3 \\
%                 \midrule
%                 ItemKNN CBF         &            16 &              +1 \\
%                 \midrule
%                 ItemKNN CFCBF       &             9 &              -2 \\
%                 \bottomrule
%             \end{tabular}
%             }
%             \caption{Carousel MAP ranking and its difference with th individual one for MovieLens10M. The fixed carousel is TopPop with the most popular genre. Kendall's $\tau$ is 0.84.}
 
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%             \centering
%             \resizebox{\columnwidth}{!}{%
%             \begin{tabular}{l|c|c|}
%                 \toprule
%                 {} & \multicolumn{2}{c|}{MAP rank} \\
%                 {} &      \begin{tabular}{@{}c@{}}Carousel \\ (TopPop new\\releases) \end{tabular} & $ \Delta $ rank \\
%                 \midrule
%                 TopPop              &            14 &               0 \\
%                 TopPop genre       &            15 &               0 \\
%                 TopPop new releases &            17 &              -1 \\
%                 \midrule
%                 UserKNN CF          &             3 &              -1 \\
%                 ItemKNN CF          &             9 &              -1 \\
%                 \palpha             &            13 &               0 \\
%                 \pbeta             &            10 &               0 \\
%                 \midrule
%                 \EASER              &             5 &               0 \\
%                 SLIM BPR            &             4 &              -1 \\
%                 SLIM EN     &             1 &               0 \\
%                 MF BPR              &            12 &               0 \\
%                 MF FunkSVD          &             7 &              +2 \\
%                 PureSVD             &             6 &               0 \\
%                 NMF                 &            11 &               0 \\
%                 IALS                &             2 &              +2 \\
%                 \midrule
%                 ItemKNN CBF         &            16 &              +1 \\
%                 \midrule
%                 ItemKNN CFCBF       &             8 &              -1 \\
%                 \bottomrule
%             \end{tabular}
%             }
%             \caption{Carousel MAP ranking and its difference with th individual one for MovieLens10M. The fixed carousel is TopPop with the new releases. Kendall's $\tau$ is 0.93.}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%             \centering
%             \resizebox{\columnwidth}{!}{%
%             \begin{tabular}{l|c|c|}
%                 \toprule
%                 {} & \multicolumn{2}{c|}{MAP rank} \\
%                 {} &      \begin{tabular}{@{}c@{}}Carousel \\ (ItemKNN CBF) \end{tabular} & $ \Delta $ rank \\
%                 \midrule
%                 TopPop              &            14 &               0 \\
%                 TopPop genre       &            15 &               0 \\
%                 TopPop new releases &            16 &               0 \\
%                 \midrule
%                 UserKNN CF          &             2 &               0 \\
%                 ItemKNN CF          &             9 &              -1 \\
%                 \palpha             &            13 &               0 \\
%                 \pbeta             &            10 &               0 \\
%                 \midrule
%                 \EASER              &             5 &               0 \\
%                 SLIM BPR            &             4 &              -1 \\
%                 SLIM EN     &             1 &               0 \\
%                 MF BPR              &            12 &               0 \\
%                 MF FunkSVD          &             8 &              +1 \\
%                 PureSVD             &             6 &               0 \\
%                 NMF                 &            11 &               0 \\
%                 IALS                &             3 &              +1 \\
%                 \midrule
%                 ItemKNN CBF         &            17 &               0 \\
%                 \midrule
%                 ItemKNN CFCBF       &             7 &               0 \\
%                 \bottomrule
                
%             \end{tabular}
%             }
%             \caption{Carousel MAP ranking and its difference with th individual one for MovieLens10M. The fixed carousel is ItemKNN CBF. Kendall's $\tau$ is 0.97.}
%     \end{minipage}
% \end{table*}


% \begin{table}[]
%     \centering
%     \footnotesize
% \begin{tabular}{l|c|cc|cc|cc|}
% \toprule
% {} & {} & \multicolumn{2}{c|}{TopPop Drama}  & \multicolumn{2}{c|}{TopPop new releases} & \multicolumn{2}{c|}{ItemKNN CBF} \\
% {} &       Individual &      Carousel & $ \Delta $ rank &      Carousel & $ \Delta $ rank &      Carousel & $ \Delta $ rank \\
% \midrule
% TopPop               &             14 &            14 &               0 &            14 &               0 &            14 &               0 \\
% TopPop Drama        &             15 &            17 &              -2 &            15 &               0 &            15 &               0 \\
% TopPop new releases  &             16 &            15 &              +1 &            17 &              -1 &            16 &               0 \\
% \midrule
% UserKNN CF    &              2 &             3 &              -1 &             3 &              -1 &             2 &               0 \\
% ItemKNN CF    &              8 &            10 &              -2 &             9 &              -1 &             9 &              -1 \\
% \palpha              &             13 &            13 &               0 &            13 &               0 &            13 &               0 \\
% \pbeta              &             10 &            11 &              -1 &            10 &               0 &            10 &               0 \\
% \midrule
% \EASER               &              5 &             6 &              -1 &             5 &               0 &             5 &               0 \\
% SLIM BPR             &              3 &             4 &              -1 &             4 &              -1 &             4 &              -1 \\
% SLIM EN      &              1 &             2 &              -1 &             1 &               0 &             1 &               0 \\
% MF BPR               &             12 &            12 &               0 &            12 &               0 &            12 &               0 \\
% MF FunkSVD           &              9 &             7 &              +2 &             7 &              +2 &             8 &              +1 \\
% PureSVD              &              6 &             5 &              +1 &             6 &               0 &             6 &               0 \\
% NMF                  &             11 &             8 &              +3 &            11 &               0 &            11 &               0 \\
% IALS                 &              4 &             1 &              +3 &             2 &              +2 &             3 &              +1 \\
% \midrule
% ItemKNN CBF   &             17 &            16 &              +1 &            16 &              +1 &            17 &               0 \\
% \midrule
% ItemKNN CFCBF &              7 &             9 &              -2 &             8 &              -1 &             7 &               0 \\
% \bottomrule
% \end{tabular}
%     \caption{Comparison of the MAP ranking under different carousels in MovieLens10M. The algorithms are used as second carousels, while the first one is TopPop Drama, TopPop new releases or the ItemKNN CBF. \nico{new releases: last 10 years}}
%     \label{tab:carousels_rank}
% \end{table}


% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel (TopPop most popular genre)} & \multicolumn{3}{c|}{MAP rank} \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &  Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop          &         0.0975 & 0.0709 & 0.0983 &        0.0646 & 0.0480 & 0.1025 &  0.1131 &             14 &            14 &               0 \\
% \midrule
% UserKNN CF      &         0.2375 & 0.2303 & 0.2804 &        0.1301 & 0.0773 & 0.1804 &  0.2437 &              2 &             3 &              -1 \\
% ItemKNN CF      &         0.1954 & 0.1780 & 0.2121 &        0.1114 & 0.0692 & 0.1552 &  0.2031 &              8 &            10 &              -2 \\
% P3alpha         &         0.1646 & 0.1414 & 0.1915 &        0.0939 & 0.0610 & 0.1400 &  0.1740 &             13 &            13 &               0 \\
% RP3beta         &         0.1886 & 0.1686 & 0.2160 &        0.1076 & 0.0670 & 0.1536 &  0.1987 &             10 &            11 &              -1 \\
% \midrule
% EASE R          &         0.2260 & 0.2070 & 0.2566 &        0.1254 & 0.0743 & 0.1702 &  0.2253 &              5 &             6 &              -1 \\
% SLIM BPR        &         0.2274 & 0.2159 & 0.2699 &        0.1272 & 0.0765 & 0.1774 &  0.2379 &              3 &             4 &              -1 \\
% SLIM EN &         0.2460 & 0.2340 & 0.2856 &        0.1372 & 0.0800 & 0.1835 &  0.2490 &              1 &             2 &              -1 \\
% \midrule
% MF BPR          &         0.1759 & 0.1502 & 0.1882 &        0.1054 & 0.0660 & 0.1473 &  0.1870 &             12 &            12 &               0 \\
% MF FunkSVD      &         0.2039 & 0.1748 & 0.2307 &        0.1244 & 0.0736 & 0.1716 &  0.2265 &              9 &             7 &              +2 \\
% PureSVD         &         0.2217 & 0.2060 & 0.2527 &        0.1275 & 0.0759 & 0.1709 &  0.2285 &              6 &             5 &              +1 \\
% NMF             &         0.1872 & 0.1613 & 0.1974 &        0.1205 & 0.0726 & 0.1613 &  0.2120 &             11 &             8 &              +3 \\
% IALS            &         0.2329 & 0.2152 & 0.2539 &        0.1357 & 0.0801 & 0.1766 &  0.2354 &              4 &             1 &              +3 \\
% \midrule
% ItemKNN CBF     &         0.0113 & 0.0052 & 0.0079 &        0.0399 & 0.0395 & 0.0807 &  0.0800 &             15 &            15 &               0 \\
% ItemKNN CFCBF   &         0.1950 & 0.1787 & 0.2151 &        0.1148 & 0.0706 & 0.1582 &  0.2079 &              7 &             9 &              -2 \\
% \bottomrule
% \end{tabular}

% }
%     \caption{Comparison of the MovieLens 10M accuracy metrics with single row and carousel evaluation, both @10. The carousel fixed is the TopPop with the most popular genre.}
%     \label{tab:ml10macc_genre}
% \end{table}



% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel (TopPop last two years)} & \multicolumn{3}{c|}{MAP rank} \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &  Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop          &         0.0975 & 0.0709 & 0.0983 &        0.0722 & 0.0357 & 0.0849 &  0.1119 &             14 &            14 &               0 \\
% \midrule
% UserKNN CF      &         0.2375 & 0.2303 & 0.2804 &        0.1287 & 0.0615 & 0.1564 &  0.2296 &              2 &             3 &              -1 \\
% ItemKNN CF      &         0.1954 & 0.1780 & 0.2121 &        0.1067 & 0.0515 & 0.1275 &  0.1817 &              8 &             9 &              -1 \\
% P3alpha         &         0.1646 & 0.1414 & 0.1915 &        0.1001 & 0.0484 & 0.1217 &  0.1717 &             13 &            13 &               0 \\
% RP3beta         &         0.1886 & 0.1686 & 0.2160 &        0.1071 & 0.0513 & 0.1297 &  0.1846 &             10 &            10 &               0 \\
% \midrule
% EASE R          &         0.2260 & 0.2070 & 0.2566 &        0.1250 & 0.0589 & 0.1475 &  0.2143 &              5 &             5 &               0 \\
% SLIM BPR        &         0.2274 & 0.2159 & 0.2699 &        0.1260 & 0.0603 & 0.1534 &  0.2241 &              3 &             4 &              -1 \\
% SLIM EN &         0.2460 & 0.2340 & 0.2856 &        0.1363 & 0.0643 & 0.1601 &  0.2360 &              1 &             1 &               0 \\
% \midrule
% MF BPR          &         0.1759 & 0.1502 & 0.1882 &        0.1023 & 0.0489 & 0.1209 &  0.1686 &             12 &            12 &               0 \\
% MF FunkSVD      &         0.2039 & 0.1748 & 0.2307 &        0.1187 & 0.0551 & 0.1418 &  0.2026 &              9 &             7 &              +2 \\
% PureSVD         &         0.2217 & 0.2060 & 0.2527 &        0.1238 & 0.0586 & 0.1452 &  0.2110 &              6 &             6 &               0 \\
% NMF             &         0.1872 & 0.1613 & 0.1974 &        0.1094 & 0.0510 & 0.1237 &  0.1755 &             11 &            11 &               0 \\
% IALS            &         0.2329 & 0.2152 & 0.2539 &        0.1320 & 0.0626 & 0.1500 &  0.2166 &              4 &             2 &              +2 \\
% \midrule
% ItemKNN CBF     &         0.0113 & 0.0052 & 0.0079 &        0.0305 & 0.0214 & 0.0428 &  0.0441 &             15 &            15 &               0 \\
% ItemKNN CFCBF   &         0.1950 & 0.1787 & 0.2151 &        0.1103 & 0.0527 & 0.1303 &  0.1862 &              7 &             8 &              -1 \\
% \bottomrule
% \end{tabular}
% }
%     \caption{Comparison of the MovieLens 10M accuracy metrics with Individual and carousel evaluation, both @10. The carousel fixed is the TopPop of the last two years. \nico{non so se servano gli improvement on TopPop oppure on TopPop years}}
%     \label{tab:ml10macc_years}
% \end{table}

% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel (ItemKNN CBF)} & Individual & Carousel &              {} \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &       \multicolumn{2}{c|}{MAP rank} & $ \Delta $ rank \\
% \midrule
% TopPop          &         0.0975 & 0.0709 & 0.0983 &        0.0541 & 0.0162 & 0.0545 &  0.0823 &             14 &            14 &               0 \\
% \midrule
% UserKNN CF      &         0.2375 & 0.2303 & 0.2804 &        0.1210 & 0.0448 & 0.1351 &  0.2146 &              2 &             2 &               0 \\
% ItemKNN CF      &         0.1954 & 0.1780 & 0.2121 &        0.0986 & 0.0350 & 0.1052 &  0.1650 &              8 &             9 &              -1 \\
% P3alpha         &         0.1646 & 0.1414 & 0.1915 &        0.0868 & 0.0300 & 0.0962 &  0.1498 &             13 &            13 &               0 \\
% RP3beta         &         0.1886 & 0.1686 & 0.2160 &        0.0986 & 0.0346 & 0.1074 &  0.1681 &             10 &            10 &               0 \\
% \midrule
% EASE R          &         0.2260 & 0.2070 & 0.2566 &        0.1168 & 0.0418 & 0.1257 &  0.1980 &              5 &             5 &               0 \\
% SLIM BPR        &         0.2274 & 0.2159 & 0.2699 &        0.1174 & 0.0432 & 0.1306 &  0.2065 &              3 &             4 &              -1 \\
% SLIM EN &         0.2460 & 0.2340 & 0.2856 &        0.1264 & 0.0462 & 0.1369 &  0.2175 &              1 &             1 &               0 \\
% \midrule
% MF BPR          &         0.1759 & 0.1502 & 0.1882 &        0.0922 & 0.0318 & 0.0970 &  0.1492 &             12 &            12 &               0 \\
% MF FunkSVD      &         0.2039 & 0.1748 & 0.2307 &        0.1059 & 0.0361 & 0.1163 &  0.1805 &              9 &             8 &              +1 \\
% PureSVD         &         0.2217 & 0.2060 & 0.2527 &        0.1146 & 0.0411 & 0.1230 &  0.1941 &              6 &             6 &               0 \\
% NMF             &         0.1872 & 0.1613 & 0.1974 &        0.0974 & 0.0327 & 0.0987 &  0.1538 &             11 &            11 &               0 \\
% IALS            &         0.2329 & 0.2152 & 0.2539 &        0.1202 & 0.0437 & 0.1257 &  0.1959 &              4 &             3 &              +1 \\
% \midrule
% ItemKNN CBF     &         0.0113 & 0.0052 & 0.0079 &        0.0057 & 0.0036 & 0.0081 &  0.0079 &             15 &            15 &               0 \\
% ItemKNN CFCBF   &         0.1950 & 0.1787 & 0.2151 &        0.1018 & 0.0361 & 0.1076 &  0.1689 &              7 &             7 &               0 \\
% \bottomrule
% \end{tabular}
% }
%     \caption{Comparison of the MovieLens 10M accuracy metrics with Individual and carousel evaluation, both @10. The carousel fixed is an ItemKNN CBF. \nico{non so se servano gli improvement on TopPop oppure on TopPop years}}
%     \label{tab:ml10macc_years}
% \end{table}

% \begin{table}[]
% \footnotesize
%     \centering
% \begin{tabular}{l|ccccccc|}
% \toprule
% {} & \multicolumn{7}{c|}{Individual} \\
% {} &        Novelty & \begin{tabular}{@{}c@{}}Div. \\ MIL\end{tabular} & \begin{tabular}{@{}c@{}}Cov. \\ Item\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Gini\end{tabular} & \begin{tabular}{@{}c@{}}Div. \\ Shannon\end{tabular} & \begin{tabular}{@{}c@{}}Cov. \\ Item \\ Correct\end{tabular} & \begin{tabular}{@{}c@{}}Avg. \\ Popularity\end{tabular} \\
% \midrule
% TopPop                 &         0.0079 &                    0.5369 &        0.0124 &         0.0020 &          4.7635 &                0.0121 &             0.8112 \\
% TopPop genre          &         0.0082 &                    0.4668 &        0.0110 &         0.0017 &          4.4866 &                0.0105 &             0.6856 \\
% TopPop new releases    &         0.0108 &                    0.0840 &        0.0078 &         0.0011 &          3.6049 &                0.0070 &             0.0951 \\
% \midrule
% UserKNN CF             &         0.0089 &                    0.9491 &        0.2464 &         0.0262 &          8.4579 &                0.1348 &             0.4535 \\
% ItemKNN CF             &         0.0086 &                    0.9029 &        0.1490 &         0.0118 &          7.3419 &                0.0913 &             0.5248 \\
% \palpha                &         0.0083 &                    0.8012 &        0.0606 &         0.0059 &          6.3318 &                0.0490 &             0.6751 \\
% \pbeta                &         0.0086 &                    0.8941 &        0.1680 &         0.0117 &          7.2875 &                0.0977 &             0.5584 \\
% \midrule
% \EASER                 &         0.0086 &                    0.9221 &        0.1020 &         0.0144 &          7.6602 &                0.0804 &             0.5326 \\
% SLIM BPR               &         0.0089 &                    0.9416 &        0.2055 &         0.0232 &          8.2771 &                0.1368 &             0.4750 \\
% SLIM EN        &         0.0090 &                    0.9491 &        0.2477 &         0.0294 &          8.5653 &                0.1799 &             0.4567 \\
% MF BPR                 &         0.0088 &                    0.9348 &        0.2040 &         0.0217 &          8.1467 &                0.1304 &             0.4957 \\
% MF FunkSVD             &         0.0094 &                    0.9762 &        0.1866 &         0.0460 &          9.3491 &                0.1597 &             0.3533 \\
% PureSVD                &         0.0088 &                    0.9428 &        0.0885 &         0.0174 &          7.9644 &                0.0846 &             0.4865 \\
% NMF                    &         0.0091 &                    0.9591 &        0.1060 &         0.0236 &          8.4094 &                0.0983 &             0.3826 \\
% IALS                   &         0.0090 &                    0.9629 &        0.1676 &         0.0300 &          8.7295 &                0.1584 &             0.4255 \\
% \midrule
% ItemKNN CBF &         0.0134 &                    0.9680 &        0.4663 &         0.0511 &          9.3030 &                0.0485 &             0.0692 \\
% \midrule
% ItemKNN CFCBF  &         0.0087 &                    0.9236 &        0.2078 &         0.0156 &          7.7111 &                0.1129 &             0.5047 \\
% \bottomrule
% \end{tabular}

%     \caption{MovieLens 10M beyond accuracy metrics according to Individual and Carousel evaluation.}
%     \label{tab:ml10mbeyondacc}
% \end{table}




% \begin{figure*}[]
%     \centering
%     \begin{minipage}{.49\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{images/MovieLens10M_subplot_beyond_acc_MAP_deg_2.pdf}
%         \caption{Plot of the MAP (Individual and carousel evaluation) of collaborative algorithms on MovieLens10M with respect to novelty and diversity metrics.\mf{provare a fare plot con MAP individual e carousel suli assi, colore/dimensione del punto diversity}}
%         \label{fig:ml10m_plots}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.49\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth]{images/Movielens10M_subplot_beyond_acc_NDCG_deg_2.pdf}
%         \caption{Plot of the NDCG (Individual and carousel 2D evaluation) of collaborative algorithms on MovieLens10M with respect to novelty and diversity metrics.}
%         \label{fig:ml10m_ndcg_plots}
%     \end{minipage}
% \end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{images/ml10m_ranking_plot_thres_1.pdf}
%     \caption{Major differences in the ranking of algorithms according to the MAP evaluated in the two different modalities for MovieLens 10M.
%     \nico{da capire quali algoritmi selezionale}}
%     \label{fig:ml10m_ranking}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{images/Ranking comparato.png}
%     \caption{Major differences in the ranking of algorithms according to the MAP evaluated in the two different modalities for MovieLens 10M.
%     \nico{da capire quali algoritmi selezionale}}
%     \label{fig:ml10m_ranking}
% \end{figure}

% \begin{table}[]
%     \footnotesize
%     \centering
%         \begin{tabular}{lccc}
%             {} &  NDCG ranking &  NDCG 2D carousel ranking &  $ \Delta $ rank \\
%             \midrule
%             SLIM EN      &             1 &                         1 &                0 \\
%             UserKNN CF cosine    &             2 &                         2 &                0 \\
%             IALS                 &             5 &                         3 &                +2 \\
%             SLIM BPR             &             3 &                         4 &               -1 \\
%             MF FunkSVD           &             7 &                         5 &                +2 \\
%             PureSVD              &             6 &                         6 &                0 \\
%             EASE R               &             4 &                         7 &               -3 \\
%             NMF                  &            11 &                         8 &                +3 \\
%             ItemKNN CFCBF cosine &             9 &                         9 &                0 \\
%             ItemKNN CF cosine    &            10 &                        10 &                0 \\
%             RP3beta              &             8 &                        11 &               -3 \\
%             MF BPR               &            13 &                        12 &                +1 \\
%             P3alpha              &            12 &                        13 &               -1 \\
%             ItemKNN CBF cosine   &            15 &                        14 &                +1 \\
%             TopPop               &            14 &                        15 &               -1 \\
%             \bottomrule
%         \end{tabular}

%     \caption{Differences in the ranking of algorithms according to the NDCG evaluated in the two different modalities for MovieLens 10M. For the carousel evaluation, NDCG 2D is considered. }
%     \label{tab:}
% \end{table}




% \begin{minipage}{.35\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{images/carousels_page_schema.pdf}
%         \captionof{figure}{prova}
% \end{minipage}
% \hfill
% \begin{table}[]
%         \centering
%         \resizebox{\columnwidth}{!}{%
%                     \begin{tabular}{l|c|cc|cc|}
%                         \toprule
%                         {} & Individual & \multicolumn{2}{c|}{Carousel (TopPop)} & \multicolumn{2}{c|}{Carousel (Big page)} \\
%                         {} &      NDCG rank &        NDCG 2D rank & $ \Delta $ rank &      NDCG 2D rank & $ \Delta $ rank \\
%                         \midrule
%                         TopPop               &             14 &                  17 &              -3 &                17 &              -3 \\
%                         TopPop genre        &             15 &                  15 &               0 &                17 &              -2 \\
%                         TopPop new releases  &             16 &                  14 &              +2 &                17 &              -1 \\
%                         \midrule
%                         UserKNN CF    &              2 &                   2 &               0 &                 3 &              -1 \\
%                         ItemKNN CF    &             10 &                  10 &               0 &                10 &               0 \\
%                         \palpha              &             12 &                  13 &              -1 &                13 &              -1 \\
%                         \pbeta              &              8 &                  11 &              -3 &                11 &              -3 \\
%                         \midrule
%                         \EASER               &              4 &                   7 &              -3 &                 8 &              -4 \\
%                         SLIM BPR             &              3 &                   4 &              -1 &                 5 &              -2 \\
%                         SLIM EN      &              1 &                   1 &               0 &                 1 &               0 \\
%                         MF BPR               &             13 &                  12 &              +1 &                12 &              +1 \\
%                         MF FunkSVD           &              7 &                   5 &              +2 &                 4 &              +3 \\
%                         PureSVD              &              6 &                   6 &               0 &                 7 &              -1 \\
%                         NMF                  &             11 &                   8 &              +3 &                 6 &              +5 \\
%                         IALS                 &              5 &                   3 &              +2 &                 2 &              +3 \\
%                         \midrule
%                         ItemKNN CBF   &             17 &                  16 &              +1 &                17 &               0 \\
%                         \midrule
%                         ItemKNN CFCBF &              9 &                   9 &               0 &                 9 &               0 \\
%                         \bottomrule
%                     \end{tabular}
%                     \caption{prova2}
%         }
% \end{table}


% \begin{table}[]
%     \footnotesize
%     \centering
%         \begin{tabular}{l|c|cc|cc|}
% \toprule
% {} & Individual & \multicolumn{2}{c|}{Carousel (TopPop)} & \multicolumn{2}{c|}{Carousel (Big page)} \\
% {} &      NDCG rank &        NDCG 2D rank & $ \Delta $ rank &      NDCG 2D rank & $ \Delta $ rank \\
% \midrule
% TopPop               &             14 &                  17 &              -3 &                17 &              -3 \\
% TopPop Drama        &             15 &                  15 &               0 &                17 &              -2 \\
% TopPop new releases  &             16 &                  14 &              +2 &                17 &              -1 \\
% \midrule
% UserKNN CF    &              2 &                   2 &               0 &                 3 &              -1 \\
% ItemKNN CF    &             10 &                  10 &               0 &                10 &               0 \\
% \palpha              &             12 &                  13 &              -1 &                13 &              -1 \\
% \pbeta              &              8 &                  11 &              -3 &                11 &              -3 \\
% \midrule
% \EASER               &              4 &                   7 &              -3 &                 8 &              -4 \\
% SLIM BPR             &              3 &                   4 &              -1 &                 5 &              -2 \\
% SLIM EN      &              1 &                   1 &               0 &                 1 &               0 \\
% MF BPR               &             13 &                  12 &              +1 &                12 &              +1 \\
% MF FunkSVD           &              7 &                   5 &              +2 &                 4 &              +3 \\
% PureSVD              &              6 &                   6 &               0 &                 7 &              -1 \\
% NMF                  &             11 &                   8 &              +3 &                 6 &              +5 \\
% IALS                 &              5 &                   3 &              +2 &                 2 &              +3 \\
% \midrule
% ItemKNN CBF   &             17 &                  16 &              +1 &                17 &               0 \\
% \midrule
% ItemKNN CFCBF &              9 &                   9 &               0 &                 9 &               0 \\
% \bottomrule
% \end{tabular}

%     \caption{Differences in the ranking of algorithms according to the NDCG for MovieLens 10M evaluated with different carousels. For the carousel evaluation, NDCG 2D is considered. Fixed carousels considered are simple TopPop and a more complex page formed of TopPop, TopPop with genre, TopPop new releases, and ItemKNN CBF. \nico{TODO controllare}}
%     \label{tab:}
% \end{table}

% \begin{table}[]
%     \footnotesize
%     \centering
% \begin{tabular}{l|cc|c|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{TopPop carousel} & \multicolumn{3}{c|}{Big page} \\
% {} &            NDCG & NDCG 2D & $ \Delta $ rank &     NDCG & NDCG 2D & $ \Delta $ rank \\
% \midrule
% TopPop               &              17 &      17 &               0 &       17 &      17 &               0 \\
% TopPop Drama        &              14 &      14 &               0 &       17 &      17 &               0 \\
% TopPop new releases  &              16 &      16 &               0 &       17 &      17 &               0 \\
% \midrule
% UserKNN CF    &               2 &       2 &               0 &        2 &       2 &               0 \\
% ItemKNN CF    &              10 &      10 &               0 &       10 &      10 &               0 \\
% \palpha              &              13 &      13 &               0 &       13 &      13 &               0 \\
% \pbeta              &              11 &      11 &               0 &       11 &      11 &               0 \\
% \midrule
% \EASER               &               7 &       7 &               0 &        8 &       8 &               0 \\
% SLIM BPR             &               4 &       4 &               0 &        5 &       4 &              +1 \\
% SLIM EN      &               1 &       1 &               0 &        1 &       1 &               0 \\
% MF BPR               &              12 &      12 &               0 &       12 &      12 &               0 \\
% MF FunkSVD           &               5 &       5 &               0 &        4 &       5 &              -1 \\
% PureSVD              &               6 &       6 &               0 &        6 &       6 &               0 \\
% NMF                  &               8 &       8 &               0 &        7 &       7 &               0 \\
% IALS                 &               3 &       3 &               0 &        3 &       3 &               0 \\
% \midrule
% ItemKNN CBF   &              15 &      15 &               0 &       17 &      17 &               0 \\
% \midrule
% ItemKNN CFCBF &               9 &       9 &               0 &        9 &       9 &               0 \\
% \bottomrule
% \end{tabular}

%     \caption{Differences in the ranking of algorithms according to the NDCG for MovieLens 10M evaluated with different carousels. For the carousel evaluation, NDCG 2D is considered. Fixed carousels considered are simple TopPop and a more complex page formed of TopPop, TopPop with genre, TopPop new releases, and ItemKNN CBF. \nico{TODO provare con big page reversed}}
%     \label{tab:}
% \end{table}



% \begin{table}[]
%     \footnotesize
%     \centering
% \begin{tabular}{l|cc|c|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{TopPop carousel} & \multicolumn{3}{c|}{Big page} \\
% {} &            NDCG & NDCG 2D & $ \Delta $ rank &     NDCG & NDCG 2D & $ \Delta $ rank \\
% \midrule
% TopPop               &              17 &      17 &               0 &       17 &      17 &               0 \\
% TopPop Drama        &              14 &      14 &               0 &       17 &      17 &               0 \\
% TopPop new releases  &              16 &      16 &               0 &       17 &      17 &               0 \\
% \midrule
% UserKNN CF    &               2 &       2 &               0 &        2 &       2 &               0 \\
% ItemKNN CF    &              10 &      10 &               0 &       10 &      10 &               0 \\
% \palpha              &              13 &      13 &               0 &       13 &      13 &               0 \\
% \pbeta              &              11 &      11 &               0 &       11 &      11 &               0 \\
% \midrule
% \EASER               &               7 &       7 &               0 &        8 &       8 &               0 \\
% SLIM BPR             &               4 &       4 &               0 &        5 &       4 &              +1 \\
% SLIM EN      &               1 &       1 &               0 &        1 &       1 &               0 \\
% MF BPR               &              12 &      12 &               0 &       12 &      12 &               0 \\
% MF FunkSVD           &               5 &       5 &               0 &        4 &       5 &              -1 \\
% PureSVD              &               6 &       6 &               0 &        6 &       6 &               0 \\
% NMF                  &               8 &       8 &               0 &        7 &       7 &               0 \\
% IALS                 &               3 &       3 &               0 &        3 &       3 &               0 \\
% \midrule
% ItemKNN CBF   &              15 &      15 &               0 &       17 &      17 &               0 \\
% \midrule
% ItemKNN CFCBF &               9 &       9 &               0 &        9 &       9 &               0 \\
% \bottomrule
% \end{tabular}

%     \caption{Differences in the ranking of algorithms according to the NDCG for MovieLens 10M evaluated with different carousels. For the carousel evaluation, NDCG 2D is considered. Fixed carousels considered are simple TopPop and a more complex page formed of TopPop new releases, ItemKNN CBF, TopPop with genre, and TopPop. \nico{Big page reversed, inserire anche i valori assoluti}}
%     \label{tab:}
% \end{table}



% \begin{table}[]
%     \centering
%         \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|c|cc|c|}
% \toprule
% {} & \multicolumn{2}{c|}{TopPop} & \multicolumn{2}{c|}{Big page} & \multicolumn{3}{c|}{TopPop}  & \multicolumn{3}{c|}{Big page} \\
% {} &   NDCG & NDCG 2D &            NDCG & NDCG 2D & NDCG rank & NDCG 2D rank & $ \Delta $ rank &       NDCG rank & NDCG 2D rank & $ \Delta $ rank \\
% \midrule
% TopPop               & 0.0983 &  0.0946 &          0.0573 &  0.0860 &        17 &           17 &               0 &              17 &           17 &               0 \\
% TopPop Drama        & 0.1109 &  0.1141 &          0.0573 &  0.0860 &        14 &           14 &               0 &              17 &           17 &               0 \\
% TopPop new releases  & 0.1007 &  0.0986 &          0.0573 &  0.0860 &        16 &           16 &               0 &              17 &           17 &               0 \\
% \midrule
% UserKNN CF    & 0.1911 &  0.2492 &          0.1157 &  0.1819 &         2 &            2 &               0 &               2 &            2 &               0 \\
% ItemKNN CF    & 0.1662 &  0.2093 &          0.0997 &  0.1558 &        10 &           10 &               0 &              10 &           10 &               0 \\
% \palpha              & 0.1451 &  0.1710 &          0.0858 &  0.1323 &        13 &           13 &               0 &              13 &           13 &               0 \\
% \pbeta              & 0.1632 &  0.2035 &          0.0975 &  0.1518 &        11 &           11 &               0 &              11 &           11 &               0 \\
% \midrule
% \EASER               & 0.1799 &  0.2293 &          0.1082 &  0.1682 &         7 &            7 &               0 &               8 &            8 &               0 \\
% SLIM BPR             & 0.1868 &  0.2414 &          0.1133 &  0.1780 &         4 &            4 &               0 &               5 &            4 &              +1 \\
% SLIM EN      & 0.1931 &  0.2530 &          0.1173 &  0.1837 &         1 &            1 &               0 &               1 &            1 &               0 \\
% \midrule
% MF BPR               & 0.1581 &  0.1932 &          0.0948 &  0.1469 &        12 &           12 &               0 &              12 &           12 &               0 \\
% MF FunkSVD           & 0.1859 &  0.2373 &          0.1141 &  0.1771 &         5 &            5 &               0 &               4 &            5 &              -1 \\
% PureSVD              & 0.1824 &  0.2357 &          0.1099 &  0.1715 &         6 &            6 &               0 &               6 &            6 &               0 \\
% NMF                  & 0.1792 &  0.2281 &          0.1094 &  0.1704 &         8 &            8 &               0 &               7 &            7 &               0 \\
% IALS                 & 0.1895 &  0.2446 &          0.1157 &  0.1808 &         3 &            3 &               0 &               3 &            3 &               0 \\
% \midrule
% ItemKNN CBF   & 0.1022 &  0.1007 &          0.0573 &  0.0860 &        15 &           15 &               0 &              17 &           17 &               0 \\
% \midrule
% ItemKNN CFCBF & 0.1696 &  0.2148 &          0.1022 &  0.1597 &         9 &            9 &               0 &               9 &            9 &               0 \\
% \bottomrule
% \end{tabular}
% }
%     \caption{Differences in the ranking of algorithms according to the NDCG for MovieLens 10M evaluated with different carousels. For the carousel evaluation, NDCG 2D is considered. Fixed carousels considered are simple TopPop and a more complex page formed of TopPop new releases, ItemKNN CBF, TopPop with genre, and TopPop. \nico{Valori assoluti inseriti}}
%     \label{tab:}
% \end{table}





% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%

%     \begin{tabular}{l|ccc|cccc|cc|cc|c|}
%         \toprule
%         {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on TopPop} &       \multicolumn{3}{c|}{MAP rank}      \\
%         {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
%         \midrule
%         TopPop             &         0.0054 & 0.0033 & 0.0071 &        0.0027 & 0.0029 & 0.0071 &  0.0064 &                  0.00\% &                  0.00\% &             10 &            10 &               0 \\
%         \midrule
%         UserKNN CF         &         0.0840 & 0.0895 & 0.1426 &        0.0433 & 0.0190 & 0.0706 &  0.1056 &              +2641.10\% &               +544.16\% &              4 &             4 &               0 \\
%         ItemKNN CF         &         0.0840 & 0.0912 & 0.1428 &        0.0432 & 0.0193 & 0.0705 &  0.1056 &              +2694.89\% &               +555.88\% &              3 &             3 &               0 \\
%         \palpha            &         0.0845 & 0.0875 & 0.1406 &        0.0432 & 0.0189 & 0.0702 &  0.1041 &              +2579.26\% &               +540.53\% &              5 &             5 &               0 \\
%         \pbeta            &         0.0962 & 0.1047 & 0.1589 &        0.0497 & 0.0224 & 0.0787 &  0.1177 &              +3108.73\% &               +659.34\% &              2 &             2 &               0 \\
%         \midrule
%         \EASER             &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
%         SLIM BPR           &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
%         SLIM EN    &         0.1066 & 0.1160 & 0.1758 &        0.0544 & 0.0244 & 0.0861 &  0.1291 &              +3452.36\% &               +728.80\% &              1 &             1 &               0 \\
%         MF BPR             &         0.0491 & 0.0442 & 0.0785 &        0.0258 & 0.0110 & 0.0430 &  0.0610 &              +1254.31\% &               +273.28\% &              9 &             9 &               0 \\
%         MF FunkSVD         &         0.0543 & 0.0486 & 0.0868 &        0.0293 & 0.0126 & 0.0493 &  0.0696 &              +1387.63\% &               +326.23\% &              8 &             8 &               0 \\
%         PureSVD            &         0.0682 & 0.0626 & 0.1061 &        0.0368 & 0.0149 & 0.0571 &  0.0826 &              +1818.08\% &               +404.18\% &              6 &             6 &               0 \\
%         NMF                &         0.0578 & 0.0510 & 0.0883 &        0.0316 & 0.0127 & 0.0491 &  0.0700 &              +1463.37\% &               +332.28\% &              7 &             7 &               0 \\
%         IALS               &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
%         \bottomrule
%     \end{tabular}

%     }
%       \caption{Comparison of the Spotify accuracy metrics with single row and carousel evaluation, both @10. For each evaluation mode, the MAP difference with the base model (TopPop) is shown for each algorithm.}
%     \label{tab:spotify_acc}
% \end{table}



% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on TopPop} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop              &         0.0984 & 0.0617 & 0.0606 &        0.0492 & 0.0403 & 0.0606 &  0.0614 &                  0.00\% &                  0.00\% &             11 &            11 &               0 \\
% \midrule
% UserKNN CF          &         0.2301 & 0.1906 & 0.1887 &        0.1369 & 0.0710 & 0.1305 &  0.1799 &               +209.12\% &                +76.25\% &              2 &             5 &              -3 \\
% ItemKNN CF          &         0.2026 & 0.1579 & 0.1548 &        0.1246 & 0.0656 & 0.1165 &  0.1565 &               +156.14\% &                +62.90\% &              5 &             6 &              -1 \\
% \palpha             &         0.1708 & 0.1244 & 0.1391 &        0.1010 & 0.0556 & 0.1048 &  0.1360 &               +101.74\% &                +38.11\% &             10 &            10 &               0 \\
% \pbeta             &         0.1878 & 0.1410 & 0.1613 &        0.1179 & 0.0628 & 0.1192 &  0.1607 &               +128.76\% &                +55.84\% &              8 &             7 &              +1 \\
% \midrule
% \EASER              &         0.2444 & 0.2014 & 0.2025 &        0.1448 & 0.0747 & 0.1353 &  0.1886 &               +226.64\% &                +85.34\% &              1 &             3 &              -2 \\
% SLIM BPR            &         0.2019 & 0.1512 & 0.1626 &        0.1175 & 0.0622 & 0.1177 &  0.1540 &               +145.27\% &                +54.50\% &              7 &             8 &              -1 \\
% SLIM EN     &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
% MF BPR              &         0.1753 & 0.1271 & 0.1260 &        0.1139 & 0.0618 & 0.1062 &  0.1375 &               +106.22\% &                +53.39\% &              9 &             9 &               0 \\
% MF FunkSVD          &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
% PureSVD             &         0.2343 & 0.1893 & 0.1920 &        0.1469 & 0.0765 & 0.1347 &  0.1876 &               +207.12\% &                +89.89\% &              3 &             2 &              +1 \\
% NMF                 &         0.2131 & 0.1658 & 0.1695 &        0.1377 & 0.0724 & 0.1265 &  0.1736 &               +168.87\% &                +79.83\% &              4 &             4 &               0 \\
% IALS                &         0.2062 & 0.1562 & 0.1512 &        0.1500 & 0.0787 & 0.1312 &  0.1785 &               +153.34\% &                +95.40\% &              6 &             1 &              +5 \\
% \bottomrule
% \end{tabular}


%     }
%       \caption{Comparison of the Netflix accuracy metrics with individual and carousel evaluation at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the TopPop carousel is computed with MAP. \mf{mancano SLIM e FunkSVD}}
%     \label{tab:netflix_acc}
% \end{table}


% \begin{table}[]
%     \centering
%     \footnotesize
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on TopPop} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop              &         0.0984 & 0.0617 & 0.0606 &        0.0492 & 0.0403 & 0.0606 &  0.0614 &                  0.00\% &                  0.00\% &             13 &            13 &               0 \\
% \midrule
% UserKNN CF          &         0.2301 & 0.1906 & 0.1887 &        0.1369 & 0.0710 & 0.1305 &  0.1799 &               +209.12\% &                +76.25\% &              3 &             7 &              -4 \\
% ItemKNN CF          &         0.2026 & 0.1579 & 0.1548 &        0.1246 & 0.0656 & 0.1165 &  0.1565 &               +156.14\% &                +62.90\% &              6 &             8 &              -2 \\
% \palpha             &         0.1708 & 0.1244 & 0.1391 &        0.1010 & 0.0556 & 0.1048 &  0.1360 &               +101.74\% &                +38.11\% &             12 &            12 &               0 \\
% \pbeta             &         0.1878 & 0.1410 & 0.1613 &        0.1179 & 0.0628 & 0.1192 &  0.1607 &               +128.76\% &                +55.84\% &             10 &             9 &              +1 \\
% \midrule
% \EASER              &         0.2444 & 0.2014 & 0.2025 &        0.1448 & 0.0747 & 0.1353 &  0.1886 &               +226.64\% &                +85.34\% &              2 &             4 &              -2 \\
% SLIM BPR            &         0.2019 & 0.1512 & 0.1626 &        0.1175 & 0.0622 & 0.1177 &  0.1540 &               +145.27\% &                +54.50\% &              8 &            10 &              -2 \\
% SLIM EN     &         0.2556 & 0.2115 & 0.2205 &        0.1545 & 0.0790 & 0.1468 &  0.2077 &               +242.99\% &                +96.12\% &              1 &             1 &               0 \\
% \midrule
% MF BPR              &         0.1753 & 0.1271 & 0.1260 &        0.1139 & 0.0618 & 0.1062 &  0.1375 &               +106.22\% &                +53.39\% &             11 &            11 &               0 \\
% MF FunkSVD          &         0.1991 & 0.1481 & 0.1615 &        0.1372 & 0.0724 & 0.1297 &  0.1769 &               +140.19\% &                +79.82\% &              9 &             6 &              +3 \\
% PureSVD             &         0.2343 & 0.1893 & 0.1920 &        0.1469 & 0.0765 & 0.1347 &  0.1876 &               +207.12\% &                +89.89\% &              4 &             3 &              +1 \\
% NMF                 &         0.2131 & 0.1658 & 0.1695 &        0.1377 & 0.0724 & 0.1265 &  0.1736 &               +168.87\% &                +79.83\% &              5 &             5 &               0 \\
% IALS                &         0.2062 & 0.1562 & 0.1512 &        0.1500 & 0.0787 & 0.1312 &  0.1785 &               +153.34\% &                +95.40\% &              7 &             2 &              +5 \\
% \bottomrule
% \end{tabular}
%     }
%       \caption{Comparison of the Netflix accuracy metrics with individual and carousel evaluation at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the TopPop carousel is computed with MAP. \nico{qui si potrebbe riassumere la tabella in testo, tabella lasciata nel repo} \nico{questo si puo' applicare anche a Spotify.}}
%     \label{tab:netflix_acc}
% \end{table}


% \nico{spotify table}
% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cccc|cc|cc|c|}
% \toprule
% {} & \multicolumn{3}{c|}{Individual} & \multicolumn{4}{c|}{Carousel} &  \multicolumn{2}{c|}{Improvement on TopPop} &       \multicolumn{3}{c|}{MAP rank}      \\
% {} &      PREC &    MAP &   NDCG &     PREC &    MAP &   NDCG & NDCG 2D &     Individual &           Carousel & Individual & Carousel & $ \Delta $ rank \\
% \midrule
% TopPop             &         0.0054 & 0.0033 & 0.0071 &        0.0027 & 0.0029 & 0.0071 &  0.0064 &                  0.00\% &                  0.00\% &             11 &            11 &               0 \\
% \midrule
% UserKNN CF         &         0.0840 & 0.0895 & 0.1426 &        0.0433 & 0.0190 & 0.0706 &  0.1056 &              +2641.10\% &               +544.16\% &              4 &             4 &               0 \\
% ItemKNN CF         &         0.0840 & 0.0912 & 0.1428 &        0.0432 & 0.0193 & 0.0705 &  0.1056 &              +2694.89\% &               +555.88\% &              3 &             3 &               0 \\
% \palpha            &         0.0845 & 0.0875 & 0.1406 &        0.0432 & 0.0189 & 0.0702 &  0.1041 &              +2579.26\% &               +540.53\% &              5 &             5 &               0 \\
% \pbeta            &         0.0962 & 0.1047 & 0.1589 &        0.0497 & 0.0224 & 0.0787 &  0.1177 &              +3108.73\% &               +659.34\% &              2 &             2 &               0 \\
% \midrule
% \EASER             &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
% SLIM BPR           &         0.0768 & 0.0778 & 0.1290 &        0.0404 & 0.0174 & 0.0665 &  0.0982 &              +2282.04\% &               +489.66\% &              6 &             6 &               0 \\
% SLIM EN    &         0.1066 & 0.1160 & 0.1758 &        0.0544 & 0.0244 & 0.0861 &  0.1291 &              +3452.36\% &               +728.80\% &              1 &             1 &               0 \\
% \midrule
% MF BPR             &         0.0491 & 0.0442 & 0.0785 &        0.0258 & 0.0110 & 0.0430 &  0.0610 &              +1254.31\% &               +273.28\% &             10 &            10 &               0 \\
% MF FunkSVD         &         0.0543 & 0.0486 & 0.0868 &        0.0293 & 0.0126 & 0.0493 &  0.0696 &              +1387.63\% &               +326.23\% &              9 &             9 &               0 \\
% PureSVD            &         0.0682 & 0.0626 & 0.1061 &        0.0368 & 0.0149 & 0.0571 &  0.0826 &              +1818.08\% &               +404.18\% &              7 &             7 &               0 \\
% NMF                &         0.0578 & 0.0510 & 0.0883 &        0.0316 & 0.0127 & 0.0491 &  0.0700 &              +1463.37\% &               +332.28\% &              8 &             8 &               0 \\
% IALS               &            - &    - &    - &           - &    - &    - &     - &                     - &                     - &              - &             - &             - \\
% \bottomrule
% \end{tabular}

%     }
%       \caption{Comparison of the Spotify accuracy metrics with individual and carousel evaluation at recommendation list length of 10. Note that in the carousel evaluation there will be two recommendation lists. The improvement over the TopPop carousel is computed with MAP. The results for two models are missing, \EASER because the original implementation required too much RAM and IALS due to the very high training time on this dataset.}
%     \label{tab:spotify_acc}
% \end{table}











% \begin{table}[h]
% 	\begin{minipage}{0.50\linewidth}
% 		\centering
% 		\footnotesize
% 		\resizebox{\columnwidth}{!}{%
%         \begin{tabular}{l|cc|cc|}
%         \toprule
%         {} & \multicolumn{2}{c|}{TopPop} & \multicolumn{2}{c|}{Long page}  \\
%         {} &   NDCG & NDCG 2D &            NDCG & NDCG 2D  \\
%         \midrule
%         TopPop               & 0.0983 &  0.0946 &          0.0573 &  0.0860  \\
%         TopPop Drama        & 0.1109 &  0.1141 &          0.0573 &  0.0860  \\
%         TopPop new releases  & 0.1007 &  0.0986 &          0.0573 &  0.0860  \\
%         \midrule
%         UserKNN CF    & 0.1911 &  0.2492 &          0.1157 &  0.1819          \\
%         ItemKNN CF    & 0.1662 &  0.2093 &          0.0997 &  0.1558         \\
%         \palpha              & 0.1451 &  0.1710 &          0.0858 &  0.1323          \\
%         \pbeta              & 0.1632 &  0.2035 &          0.0975 &  0.1518       \\
%         \midrule
%         \EASER               & 0.1799 &  0.2293 &          0.1082 &  0.1682        \\
%         SLIM BPR             & 0.1868 &  0.2414 &          0.1133 &  0.1780       \\
%         SLIM EN      & 0.1931 &  0.2530 &          0.1173 &  0.1837        \\
%         \midrule
%         MF BPR               & 0.1581 &  0.1932 &          0.0948 &  0.1469      \\
%         MF FunkSVD           & 0.1859 &  0.2373 &          0.1141 &  0.1771        \\
%         PureSVD              & 0.1824 &  0.2357 &          0.1099 &  0.1715         \\
%         NMF                  & 0.1792 &  0.2281 &          0.1094 &  0.1704       \\
%         IALS                 & 0.1895 &  0.2446 &          0.1157 &  0.1808         \\
%         \midrule
%         ItemKNN CBF   & 0.1022 &  0.1007 &          0.0573 &  0.0860   \\
%         \midrule
%         ItemKNN CFCBF & 0.1696 &  0.2148 &          0.1022 &  0.1597  \\
%         \bottomrule
%         \end{tabular}
%         }
% % 		\caption{Ranking quality comparison.}
% % 		\label{tab:ndcg_vs_ndcg2d_long_page}
%     \end{minipage}\hfill
% 	\begin{minipage}{0.45\linewidth}
% 		\centering
% 		\includegraphics[width=0.8\textwidth]{images/carousels_page_schema.pdf}
% % 		\captionof{figure}{Long Page carousel layout.}
% % 		\label{fig:example_long_page}
% 	\end{minipage}
% 	\caption{Comparison of the NDCG and NDCG2D metrics in two carousel evaluation for the MovieLens 10M dataset. In the TopPop case the first carousel is a TopPop and the second is the evaluated model. In the Long Page case the carousels are, in order from the first: TopPop new releases, ItemKNN CBF, TopPop Drama, TopPop and the evaluated model.}
% 	\label{tab:ndcg_vs_ndcg2d_long_page}
% \end{table}


% \subsection{Discussion on NDCG2D}
% As described in Section \ref{sec:two_dim_NDCG},
% %and as visualized in Figure \ref{fig:dcg_vs_dcg2d_heatmap}
% the two-dimension NDCG2D will be less penalizing of correct recommendations which appear in carousels other than the first one. This means that it is expected that in a setting where recommendation lists with high accuracy are provided after other lists with less accuracy, the NDCG2D will have a higher value than NDCG. As the complexity of the page increases and the number of carousels grow, the NDCG2D will be able to measure the difference between different configurations, whereas the NDCG applied on the single concatenated recommendation list will discount the lower carousels to such an extent that differences due to correct recommendations may become difficult to distinguish from other sources of experimental stochasticity and noise.
% By looking at Table \ref{tab:ml10macc} 
% %and \ref{tab:netflix_acc}
% %and \ref{tab:spotify_acc}
% we can see how the NDCG and NDCG2D of TopPop are very similar, as expected. Their difference is due to the different way the IDCG is computed. We can also see that NDCG2D is much higher than NDCG for most of the personalized algorithms, this is due to the lower penalization of the correct recommendations in the second carousel. 
% Table \ref{tab:ndcg_vs_ndcg2d_long_page} compares NDCG and NDCG2D in the previous TopPop carousel setting as well as in a more complex setting where the page contains 5 carousels. 
% We can see that while in the TopPop setting the difference between the two metrics is in the range of 30\%, in the longer page becomes as high as 60\%.
% \nico{r1 si chiede perché il comparison su accuracy è stato fatto per tutti i dataset mentre MAP ranking (tab3) e NDCGvsNDCG2D (tab6) solo per ML10M}
% \nico{La teniamo questa discussione su ndcg2d?}



% \begin{table}[]
% \footnotesize
%     \centering
%         %\resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|cc|cc|}
% \toprule
% {} & \multicolumn{2}{c|}{TopPop} & \multicolumn{2}{c|}{Big page}  \\
% {} &   NDCG & NDCG 2D &            NDCG & NDCG 2D  \\
% \midrule
% TopPop               & 0.0983 &  0.0946 &          0.0573 &  0.0860  \\
% TopPop Drama        & 0.1109 &  0.1141 &          0.0573 &  0.0860  \\
% TopPop new releases  & 0.1007 &  0.0986 &          0.0573 &  0.0860  \\
% \midrule
% UserKNN CF    & 0.1911 &  0.2492 &          0.1157 &  0.1819          \\
% ItemKNN CF    & 0.1662 &  0.2093 &          0.0997 &  0.1558         \\
% \palpha              & 0.1451 &  0.1710 &          0.0858 &  0.1323          \\
% \pbeta              & 0.1632 &  0.2035 &          0.0975 &  0.1518       \\
% \midrule
% \EASER               & 0.1799 &  0.2293 &          0.1082 &  0.1682        \\
% SLIM BPR             & 0.1868 &  0.2414 &          0.1133 &  0.1780       \\
% SLIM EN      & 0.1931 &  0.2530 &          0.1173 &  0.1837        \\
% \midrule
% MF BPR               & 0.1581 &  0.1932 &          0.0948 &  0.1469      \\
% MF FunkSVD           & 0.1859 &  0.2373 &          0.1141 &  0.1771        \\
% PureSVD              & 0.1824 &  0.2357 &          0.1099 &  0.1715         \\
% NMF                  & 0.1792 &  0.2281 &          0.1094 &  0.1704       \\
% IALS                 & 0.1895 &  0.2446 &          0.1157 &  0.1808         \\
% \midrule
% ItemKNN CBF   & 0.1022 &  0.1007 &          0.0573 &  0.0860   \\
% \midrule
% ItemKNN CFCBF & 0.1696 &  0.2148 &          0.1022 &  0.1597  \\
% \bottomrule
% \end{tabular}
% %}
%     \caption{Differences in the ranking of algorithms according to the NDCG for MovieLens 10M evaluated with different carousels. For the carousel evaluation, NDCG 2D is considered. Fixed carousels considered are simple TopPop and a more complex page formed of TopPop new releases, ItemKNN CBF, TopPop with genre, and TopPop. }
%     \label{tab:}
% \end{table}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{images/carousels_page_schema.pdf}
%     \caption{A more complex page considered for NDCG2D evaluation. The fixed carousels are TopPop, TopPop drama, TopPop new releases, and ItemKNN CBF.  \nico{controllare caption} \nico{mettere a fianco della NDCG2D table} \nico{controllare che l'esempio sia consistente con la pagina valutata}
%     }
%     \label{fig:example_complex_page}
% \end{figure}


% ---------------------------------------- DISCUSSIONE RISULTATI CON TOPPOP COME CAROSELLO FISSATO----------------------------------------------


% Looking at the results,
% we can see that almost all algorithms have a recommendation quality between two and three times better than TopPop under the traditional individual evaluation. The best performing algorithms are SLIM, UserKNN and IALS.
% For the carousel evaluation, the difference of MAP of the algorithms over the TopPop carousel is still wide but smaller. This is because the personalized models only fill half of the entire set of recommendations provided to the user and the evaluation only measures the \emph{new} correct recommendations the personalized model allows. 

% As a general trend we can see that the relative performance of the models differ, resulting in changes to the ranking of the algorithms in the two evaluation modes. Some models, in this case all other matrix factorization algorithms, gain 2 or 3 positions with the exception of NMF that jumps up by 8 positions becoming the 3\textsuperscript{rd} best model. On the other hand, KNNs, graph-based and item-based machine learning models tend to lose some positions. As a result, in the carousel evaluation the best algorithms are IALS, SLIM EN and NMF.
% The difference in those rankings lies in how those recommendations intersect. Algorithms which will tend to recommend popular items will be penalized in this carousel evaluation because popular items will already be present in the TopPop carousel, whereas algorithms providing accurate recommendation but involving less popular items will be advantaged. 




% ---------------------------------------- DISCUSSIONE RISULTATI CON SLIM EN COME CAROSELLO FISSATO----------------------------------------------


Based on the MAP of the individual evaluation, the best performing algorithms are SLIM, UserKNN and IALS. 
% As expected, as SLIM EN is the best performing algorithm, all the other models have a lower recommendation quality, but we can notice how this is not a good indicator of how well recommendations will intersect with the fixed SLIM EN carousel.
However, when looking at the results of the carousel evaluation, we can see that many differences emerge. For example, \palpha has an individual MAP that is 39.5\% lower than SLIM EN, while \EASER only 11.5\% lower. In the carousel evaluation instead, the improvement provided by these two algorithms is similar with \palpha being slightly better. The discrepancy between individual and carousel evaluation is even clearer if we look at the column showing the difference in the rankings of all algorithms in the two scenarios. 
As a general trend we can see that the relative performance of the models differ, resulting in several changes to the ranking of the algorithms. Some models, in this case all matrix factorization algorithms (except for PureSVD) gain several positions. NMF and MF BPR jump up by 6 positions. On the other hand, item-based machine learning models tend to lose some positions. 
As a result, in the carousel evaluation the best algorithms are IALS, FunkSVD and UserKNN.
The difference in those rankings lies in how those recommendations intersect. Algorithms which will tend to recommend items similar to the ones provided by SLIM EN will be penalized in this carousel evaluation, whereas algorithms providing accurate but different recommendations
%but involving less similar items
will be advantaged. An interesting case is \EASER, which loses 8 positions, probably because of its resemblance with the SLIM algorithm.

% Also, it is noteworthy that NDCG and NDCG2D can lead to different decisions in the carousel evaluation. 
Regarding the NDCG2D metric, we can notice how it too can lead to different decisions with respect to the standard NDCG in the carousel evaluation, though to a lesser extent.
Looking at the results in Table \ref{tab:ml10macc_slim}, we notice that the NDCG results of \EASER and Item KNN are very similar under the carousel evaluation, but NDCG2D will give a slight preference for Item KNN instead. This difference will become more marked as the page layout becomes more complex including more and longer carousels.



\section{Conclusions and Future Work}
\label{sec:conclusions}
%\nico{r1: dividi conlcusions e future work} 
This paper proposes a new offline evaluation protocol for a carousel user interface, where the recommendation quality of a model is not measured independently but rather is put into the context of other recommendation lists being already available to the users. The experimental analysis shows that the relative ranking of the personalized algorithms changes when a carousel is fixed as the first displayed to the user.
% has a reasonably good performance\nico{non so se ora vale ancora questa frase, forse direi: when a fixed carousel is available}.
This is in line with previous observations that the correlations between models have an important role to play and should be taken into account during offline evaluation as well. Further study is needed to better understand this impact. 
% As future work, an extended offline
Important future work is an online study
%should be conducted 
to measure how closely the offline carousel evaluation is able to represent the user behavior, as well as extended offline evaluation, involving a wider array of scenarios, for example sequential recommendation and also including families of models not analyzed in this paper.

% Further analysis could also be conducted including a wider array of scenarios, for example sequential recommendation and also including families of models not analyzed in this paper. 
Ultimately, the carousel evaluation protocol will allow researchers to conduct offline evaluations in these industrially relevant scenarios and open a wide number of research possibilities in studying how to combine the strength of various models and techniques to provide the user with ever more accurate and interesting recommendations.


